CARoL: Context-aware Adaptation for Robot Learning

Using Reinforcement Learning (RL) to learn new robotic tasks from scratch is often inefficient. Leveraging prior knowledge has the potential to significantly enhance learning efficiency, which, however, raises two critical challenges: how to determine the relevancy of existing knowledge and how to adaptively integrate them into learning a new task. In this paper, we propose Context-aware Adaptation for Robot Learning (CARoL), a novel framework to efficiently learn a similar but distinct new task from prior knowledge. CARoL incorporates context awareness by analyzing state transitions in system dynamics to identify similarities between the new task and prior knowledge. It then utilizes these identified similarities to prioritize and adapt specific knowledge pieces for the new task. Additionally, CARoL has a broad applicability spanning policy-based, value-based, and actor-critic RL algorithms. We validate the efficiency and generalizability of CARoL on both simulated robotic platforms and physical ground vehicles. The simulations include CarRacing and LunarLander environments, where CARoL demonstrates faster convergence and higher rewards when learning policies for new tasks. In real-world experiments, we show that CARoL enables a ground vehicle to quickly and efficiently adapt policies learned in simulation to smoothly traverse real-world off-road terrain.

==> Contents/abstract.tex <==
\begin{abstract}
    Using Reinforcement Learning (RL) to learn new robotic tasks from scratch is often inefficient. Leveraging prior knowledge has the potential to significantly enhance learning efficiency, which, however, raises two critical challenges: how to determine the relevancy of existing knowledge and how to adaptively integrate them into learning a new task. In this paper, we propose \textit{Context-aware Adaptation for Robot Learning} (CARoL), a novel framework to efficiently learn a similar but distinct new task from prior knowledge. CARoL incorporates context awareness by analyzing state transitions in system dynamics to identify similarities between the new task and prior knowledge. It then utilizes these identified similarities to prioritize and adapt specific knowledge pieces for the new task. Additionally, CARoL has a broad applicability spanning policy-based, value-based, and actor-critic RL algorithms. 
    We validate the efficiency and generalizability of CARoL on both simulated robotic platforms and physical ground vehicles. 
  Simulations include CarRacing and LunarLander environments, where CARoL demonstrates faster convergence and higher rewards when learning policies for new tasks. 
    In real-world experiments, we show that CARoL enables a ground vehicle to quickly and efficiently adapt policies learned in simulation to smoothly traverse real-world off-road terrain.
    
    
    %Reinforcement learning (RL) from scratch in new robotic tasks is often inefficient and resource-intensive. Leveraging prior knowledge can significantly enhance learning efficiency, but this raises two critical challenges: what existing knowledge to use and how to utilize it effectively. In this paper, we propose \textit{context-aware adaptation for robot learning} (CARoL), a novel framework to efficiently learn a similar but distinct new task from prior knowledge. CARoL first identifies state transitions as valuable knowledge to compare the similarities of different tasks. Then CARoL uses the similarities to prioritize learning knowledge for the new task. Additionally, CARoL extends its applicability from on-policy to off-policy RL algorithms. We further validate the efficiency and generality of our approach on simulations and the physical robotics platform. In simulations on CarRacing and LunarLander, we show that CARoL efficiently learns a policy in the new task with a faster and higher reward convergence. In real-world robotic experiments, we show that the vehicle quickly adapts to efficiently and smoothly traverse a new terrain.

    % Robots learning from scratch in new tasks is often inefficient and resource-intensive. Leveraging prior knowledge can significantly enhance learning efficiency, but this raises two critical challenges: what existing knowledge to use and how to utilize it effectively. In this paper, we propose a novel framework that identifies state transitions and policies from previously similar but distinct tasks as valuable prior knowledge. Our method leverages task similarity to distill effective policies for new tasks by integrating these priors. We validate the generality and efficiency of our approach through experiments in OpenAI environments, including CarRacing and LunarLander. Furthermore, we demonstrate its effectiveness in real-world robotic experiments, showcasing improved performance compared to baseline methods.
\end{abstract}

==> Contents/conclusion.tex <==
%\section{Limitations}






%CARoL's current limitations primarily lie in its need for asynchronous processing of context-awareness and adaptation. Specifically, CARoL cannot yet perform real-time awareness of a task's dynamic contexts. As a result, the current version of CARoL prioritizes the utilization of prior knowledge based on the overall task similarity, potentially overlooking finer details in the task. Moreover, CARoL heavily relies on solid teacher knowledge. Since CARoL's context-awareness is based on state transitions, it requires a relatively direct connection between the states and the environmental dynamics. For example, in the original CarRacing setup, the image-based observations are not strongly correlated with the task dynamics, which leads to suboptimal evaluation of knowledge relevance. Additionally, experiments reveal that CARoL exhibits oscillations during the initial phase of adaptation, further highlighting areas for improvement.


\section{Conclusion and Limitations}
In this paper, we presented CARoL. CARoL is a framework that first evaluates contextual similarities between source and target tasks based on their state transitions. Given the prior knowledge from source tasks, CARoL then performs contextual knowledge adaptation for target tasks.
A key advantage of CARoL is its broad applicability to policy-based, value-based, and actor-critic RL methods. Experimental results demonstrated that our algorithm effectively adapts to new tasks. We validated CARoL’s performance in two open-source simulated environments and on a physical robot platform, where CARoL successfully transferred prior knowledge learned in simulation to real-world off-road environments.
For future work, we aim to integrate context similarity evaluation synchronously into the adaptation process. Additionally, we plan to extend CARoL beyond single-robot adaptation to multi-agent environments, leveraging multi-agent coordination to achieve more effective context representation for task adaptation.


%which first evaluates the contextual similarities between source tasks and target tasks based on their state transition. Then, given the prior knowledge of source tasks, CARoL performs contextual knowledge adaptation for target tasks.
%A unique aspect of CARoL is its applicability to policy-based, value-based, and actor-critic-structured RL methods. Experimental results demonstrate that our algorithm can effectively adapt to new tasks. We validate CARoL's performance enhancement in two open-source simulated environments and on a physical robot platform, where CARoL successfully adapts prior knowledge learned in simulation to real-world off-road environments.
%For future work, we aim to embed context similarity evaluation synchronously into the adaptation process. Additionally, we plan to extend CARoL beyond single-robot adaptation to multi-agent environments, leveraging multi-agent coordination to achieve better context representation for task adaptation.

%We presented a framework for Context-aware Adaptation for Robot Learning (CARoL). Given prior knowledge, CARoL evaluates contextual similarities between source tasks and target tasks through their context representations and performs contextual knowledge adaptation for the new task. CARoL uses state transitions for context awareness to determine the relationship between prior knowledge and the target task, enabling the prioritization and adaptation of specific knowledge for the new task. A key enabler of CARoL is its applicability to policy-based, value-based, and even actor-critic structured RL methods. Experimental results demonstrated that our algorithm can effectively adapt to new tasks. We validated CARoL's performance enhancement in two open-source environments and further confirmed its effectiveness in physical experiments, where CARoL successfully adapted prior knowledge learned in simulation to real-world off-road terrains.

%For future work, we aim to embed context similarity evaluation synchronously into the adaptation process. Additionally, we plan to extend CARoL beyond single-robot adaptation to multi-agent environments, leveraging multi-agent communication mechanisms to achieve better context representation for task adaptation.

==> Contents/introduction.tex <==
\section{Introduction}
%\marginXW{Add References, for arxiv papers, check if they have formal accepted versions of bib.}
In recent years, Reinforcement Learning (RL) approaches have achieved remarkable success in advanced robotic control and complex task learning in dynamic environments, enabling applications across various domains, such as autonomous navigation~\cite{xiao2022motion, xu2023benchmarking}, %chiang2019learning, chen2019crowd, faust2018prm, xu2021applr, xu2024reinforcement}, 
manipulation~\cite{sun2022fully}, %ghadirzadeh2017deep, kalashnikov2018scalable, honerkamp2021learning}, 
and human-robot interaction~\cite{roveda2020model}. 
Despite these advancements, RL methods are typically computationally demanding, as they rely on repeated trial-and-error exploration to discover high-reward outcomes. 

Knowledge fusion and adaptation~\cite{ruder2017knowledge} provide promising approaches to address the inefficiency of RL.
%To address this, a promising approach is knowledge adaption, which 
They leverage knowledge (such as a learned control policy, approximated value function, etc.) from previously explored tasks to accelerate training on new tasks, eliminating the need to train from scratch for every scenario.
For example, consider a vehicle navigating highly complex off-road terrain as shown in Fig. \ref{fig:intro}. Suppose the vehicle has undergone extensive training in several existing environments, it should ideally be capable of adapting to a new type of terrain by utilizing previously learned knowledge.


Our goal is to leverage prior knowledge to enhance learning efficiency of a new task. Existing indiscriminate knowledge fusion methods~\cite{wang2021selective} do not consider (and exploit) the relationship between previous and new environments, i.e., being unaware of the environment context, even though many skills are context-specific. Instead, robots should selectively prioritize and utilize knowledge/skills that are relevant to the new task. This poses two key challenges: how to effectively quantify the relevance of existing knowledge to a new task and how to adaptively integrate it into the learning process.

%knowledge fusion methods such as multi-task reinforcement learning can guarantee performance for previously encountered scenarios but may fail in new contexts; knowledge adaption methods such as meta-learning typically lack awareness of the specific context of a new task and are unable to prioritize relevant components of prior knowledge.  
%To address this, this paper proposes a new method, Context-aware Adaptation for Robot Learning (CARoL).

%RL methods have demonstrated remarkable success in leveraging large datasets to train robots for complex tasks in dynamic environments. However, RL agent is generally initialized without any prior knowledge, it must try many largely unproductive behaviors before it discovers a high-reward outcome. The inefficiency of training for new tasks, which often requires learning from scratch that demands significant time, computational resources, and large amounts of data.
%For example, the autonomous mobile robot is deployed in unstructured, off-road environments for the search and rescue mission. Training a specific model for this task is time-cost and resource-intensive. Suppose the robot has already undergone extensive training and learning in simulation environments for navigating tasks on low-friction and high-friction off-road terrains, such as grass and rocky roads. Now, we need to navigate on an unknown terrain where neither the level of friction nor the specific type of terrain is known. Despite this, it remains a challenge that how to directly apply the learned knowledge to such unseen and specific scenarios.


%\marginXW{In general, the references need to be newer, we don't want references to be 10 years old.}
%Addressing these challenges requires knowledge fusion, where a major existing line of research lies in multi-task reinforcement learning~\cite{zhang2021survey}: Techniques such as policy distillation~\cite{rusu2015policy} and actor-mimic~\cite{parisotto2015actor} transfer knowledge from one or multiple teacher policies into a single-student policy. However, these combined policies often perform well only in previously encountered scenarios and may fail~\cite{x} \marginXW{This is an important reference. Find an appropriate one.} in new contexts, even when those contexts are closely related to the training ones.
%Another relevant approach is meta-learning~\cite{finn2017model}, which optimizes a meta-model by leveraging second-order gradients of the meta-objective to adjust the initial policy parameters for task adaptation. This enables robots to learn new tasks with less data and fewer training iterations. However, meta-models typically lack awareness of the specific context of a new task and are unable to prioritize relevant components of prior knowledge. As a result, they treat all knowledge equally and potentially reduce the efficiency of adaptation.
%\marginXW{One sentence about life long learning? Can it share the same `However' part with meta-learning?}
%In terms of quick adaptions of robot learning, existing works have explored encoding environment or robot dynamics (such as physical parameters~\cite{x} or their latent encodings~\cite{}) as part of the policy input~\cite{},
%However, identifying critical features of the environment or robot dynamics can be challenging, and some features may not be directly observable or measurable.
%\marginXW{Check the page 2, second paragraph of ref RMA ~\cite{kumar2021rma} to find relevant references here.}


\begin{figure}
    \centering
    \includegraphics[width=0.42\textwidth]{Contents/Figures/intro_v2.pdf}
    \caption{Autonomous off-road navigation: a vehicle extensively trained in (simulated) grass and concrete environments. However, its next task requires it to navigate on (real-world) unseen rocky terrain. The vehicle must effectively leverage the prior knowledge to solve this new challenge.\vspace{-1em}}
    \label{fig:intro}
\end{figure}
%\marginXW{Check captions!}

%\marginXW{This paragraph might need changes based on the revision of Sec. II.}
In this work, we propose \textit{\textbf{C}ontext-aware \textbf{A}daptation for \textbf{Ro}bot \textbf{L}earning} (CARoL), a framework that leverages context awareness to enable efficient adaptation to new tasks using prior knowledge. 
CARoL introduces a novel approach to quantify task similarities by using \textit{state transition} representations as contextual indicators, which is different from other context-awareness works that commonly use environment~\cite{kumar2021rma} or robot~\cite{yang2020multi} representations.
%Our explicate use of state transition as contextual representation is also different from the Rapid Motor Adaptation (RMA)~\cite{kumar2021rma}, which inversely estimates environmental encoding from state transitions. 
The rationale behind this choice is that the state transition is the core of a Markov Decision Process (MDP) upon which reinforcement learning is established. State transition inherently captures the combined effects of the environment and the robot, thus, is a more straightforward and comprehensive measure of task similarity, without the need of carefully choosing features from environments or robots. 
For instance, steep inclines and partially icy surfaces may differ significantly in their environmental characteristics but can produce similar state transitions such as wheel traction loss. By leveraging this shared context, control policies can be adapted in a more general and robust manner.
% control policies can be adapted more effectively.



%CARoL consists of three steps. In the first step, we focus on obtaining prior knowledge in existing environments. Unlike traditional multi-task learning, which focuses solely on training teacher policies for different tasks, our method additionally trains a state transition representation to capture the `context' of each task. 
%The second step involves evaluating contextual similarities by comparing each state transition representation with the state transition of the new task. Finally, we use the similarity to prioritize the most contextually appropriate knowledge for adaption, enabling efficient learning for the new task. Such adaption applies to policy-based, value-based and actor-critic RL algorithms.
The contributions of CARoL are threefold:
\begin{itemize}[leftmargin=*]
    \item CARoL explicitly leverages state transition to identify task-specific contextual similarity, enabling more targeted learning rather than indiscriminate fusion/adaptation of prior knowledge.
    \item CARoL has broad applicability that can be integrated into both policy-based and value-based (or combined actor-critic) RL algorithms to achieve knowledge adaptation.
    \item Our experimental study demonstrates the effectiveness of CARoL, not only in simulation environments but also through validation on physical off-road navigation tasks.
\end{itemize}


%\marginXW{Sim to real gap?}

%Knowledge can be transferable even if the terrain are significantly different. Latent features of the environment that can't be directly observed but will still be robustly captured by the state transition. 







%Multi-task reinforcement learning \cite{zhang2021survey} offers a feasible approach by enabling the mobile robot to learn end-to-end motion controls from different terrains and combine them into one single policy to address all encountered scenarios. Among the methods for multi-task reinforcement learning, policy distillation \cite{rusu2015policy} and actor-mimic \cite{parisotto2015actor} have emerged as an effective method for leveraging prior knowledge from one or multiple teacher policies to a single student policy. However, they often lack mechanisms to effectively identify and prioritize relevant components of prior knowledge in novel contexts, which poses challenges challenges in adapting to robotics tasks with similar yet different dynamics. 
%Additionally, traditional transfer learning methods are often inadequate as they lack a robust mechanism to identify and adapt relevant components of existing policies to new task contexts. MAML \cite{finn2017model} enables the robot to rapidly adapt to the new task with minimal data and training from existing tasks. However, MAML optimizes a meta-policy by leveraging second-order gradients of the meta-objective to adjust the initial policy parameters for task-specific adaptation, without explicitly considering the influence of contextual dynamics changes within the tasks.





% In recent years, data-driven approaches have significantly advanced robotic control and learning, enabling applications across various domains such as autonomous navigation, manipulation, and human-robot interaction. These methods have demonstrated remarkable success in leveraging large datasets and machine learning algorithms to train robots for complex tasks in dynamic environments. Among these advancements, reinforcement learning (RL) has further revolutionized robot learning by providing a general framework for training agents to make sequential decisions in diverse and challenging scenarios. However, RL agent is generally initialized without any prior knowledge, it must try many largely unproductive behaviors before it discovers a high-reward outcome. The inefficiency of training for new tasks, which often requires learning from scratch that demands significant time, computational resources, and large amounts of data. In contrast, humans rarely approach new tasks by learning entirely from scratch; instead, they leverage prior experiences to narrow down the search space and make informed decisions. For instance, when encountering adverse weather conditions during a flight, pilots rely on prior emergency training conducted in simulated environments, such as heavy fog, strong winds, or snowstorms. These experiences provide valuable priors that enable them to adapt to unfamiliar weather conditions efficiently, rather than relearning how to operate the aircraft under the current challenging circumstances. Similarly, for the robot learning, leveraging prior experiences can significantly enhance efficiency and adaptability.  

% Traditional transfer learning methods are often inadequate as they lack a robust mechanism to identify and adapt relevant components of existing policies to new task contexts, limiting their effectiveness in real-world robotics applications. Policy distillation has emerged as an effective method for leveraging prior experiences by transferring knowledge from one or multiple teacher policies to a single student policy. However, existing methods for policy distillation often lack mechanisms to effectively identify and prioritize relevant components of prior policies in novel contexts, especially leading to challenges in adapting to robotics tasks with significantly different dynamics. 


\begin{comment}
In this work, we propose \textit{\textbf{C}ontext-aware \textbf{A}daptation for \textbf{Ro}bot \textbf{L}earning} (CARoL), a framework that leverages context awareness by analyzing state transitions to identify and utilize similarities with prior knowledge, enabling efficient adaptation to new tasks. State transition refers to the process by which an agent moves from one state to another, driven by its action and the contextual dynamics. Our approach consists of two primary phases: the acquisition of prior knowledge and the adaptation of those learned knowledge in new target task. In the first phase, we focus on obtaining prior knowledge. Unlike traditional multi-task learning, which focuses solely on training teacher policies for different tasks, our method additionally trains a transition function to capture the contextual dynamics of each task. This transition function serves as a hidden form of prior knowledge, complementing the explicit information provided by teacher policies. The second phase involves the distillation of prior knowledge. In this stage, we utilize the prior transition functions by testing their performance in the target task and comparing the results. This comparison allows us to evaluate the similarity between the contextual dynamics of the target task and those of the tasks associated with the teacher policies. Based on this similarity, we prioritize the most relevant teacher policies for learning, enabling the agent to efficiently adapt to the target task by leveraging the most contextually appropriate knowledge.

To summarize, our contributions are threefold:
\begin{itemize}
    \item We propose the context-aware adaptation framework, which leverages state transition as prior knowledge to identify task-specific contexts, enabling more targeted learning rather than blind adaptation.
    \item Our approach generalizes the application of CARoL framework, extending its use beyond on-policy methods to include off-policy algorithms in RL.
    \XW{Consider, We explore the use of CARoL for both on-policy and off-policy algorithms.}
    \marginXW{Model policy based?}
    \item Our empirical study demonstrates the effectiveness of the proposed framework, not only in simulation environments but also through validation on the off-road autonomous mobile robot tasks.
\end{itemize}

This paper is structured as follows. Section \ref{sec:literature} summarizes the related work. In Section \ref{sec:problem}, we describe the background knowledge and problem statement. Section \ref{} firstly presents XXX, and then provides our approach of XXXX, followed by the theoretical results. Section \ref{} presents an empirical illustration of both XXXX experiments. Finally, Section \ref{} concludes and discusses the future work.
\end{comment}

==> Contents/literature.tex <==
\section{Related Work} \label{sec:literature}
%Leveraging prior knowledge is closely related to knowledge fusion, such as multi-task reinforcement learning. Learning adaptation enhances efficiency when tackling new tasks. Additionally, evaluating the relevance of existing knowledge to a new task is closely linked to context-awareness. In this section, we provide a detailed review of the relevant literature.


%Our goal is to leverage prior knowledge to enhance the learning efficiency of a net task. This is related to 

%requires knowledge fusion 

%and adaption. 

%We review existing methods in the literature that can be used for knowledge fusion and adaptation for robot learning.
%In this section, we review methods that address the learning efficiency of RL from prior knowledge.

%\marginXW{Think carefully and try to answer the question in our meeting: What are the true limitations of each type of existing method, compared with our approach.}

%\subsection{Multi-task Reinforcement Learning}

%selectively prioritize and utilize relevant prior knowledge.
%Such an indiscriminate choice limits their ability to adapt to changes in new task requirements.

%Multi-task learning aims to learn multiple tasks simultaneously, leveraging shared knowledge to improve sample efficiency and generalization in robotics and RL \cite{zhang2021survey}. \cite{wilson2007multi} introduces a hierarchical Bayesian framework for multi-task reinforcement learning to improve knowledge transfer across tasks by leveraging shared structure among related tasks. \cite{hausman2018learning} further enables robots to acquire transferable skills across a variety of tasks through learning a shared embedding space. MT-Opt \cite{kalashnikov2021mt} allows robots to learn a wide range of skills. \cite{xing2024multi} leverages shared physical dynamics to enhance sample efficiency and task performance in quadrotor control tasks. While sharing parameter across tasks can intuitively improve data efficiency, gradients from different tasks can interfere negatively with each other. One way to avoid it is to use policy distillation \cite{rusu2015policy, teh2017distral}. Actor-mimic \cite{parisotto2015actor} is also proposed in a similar idea to train a single policy by using the guidance of several expert teachers. No matter policy distillation or actor-mimic, they perform well on tasks that have already been encountered or on unseen task with known structural or dynamic similarity. However, the issue for these multi-task reinforcement learning methods in robotics is that, in most cases, the robot is unclear what kind of task it will face. When encountering an unknown task, those methods lack a mechanism or module to identify the relevant components of prior knowledge, making it difficult for the robot to adapt to dynamic changes in the task.


\subsection{Learning Adaptation for Robotics}
%To this end, various approaches have been proposed. Lifelong learning, for example, maintains a single model that evolves over time to handle all encountered tasks. This approach enables robots to continuously acquire, adapt, and transfer knowledge throughout their operational lifespan. 
By leveraging shared knowledge, multi-task learning improves sample efficiency and generalization in robotics and RL~\cite{zhang2021survey}. For example, \citet{hausman2018learning} enabled robots to acquire transferable skills across a variety of tasks through learning a shared embedding space. MT-Opt~\cite{kalashnikov2021mt} demonstrated how robots can learn a broad spectrum of skills. For quadrotor control tasks, \citet{xing2024multi} leveraged shared physical dynamics to enhance sample efficiency and task performance. 
Although parameter sharing across tasks can intuitively improve data efficiency, during the training process, gradients from different tasks can interfere negatively with each other. To mitigate this, methods such as policy distillation \cite{teh2017distral} and actor-mimic \cite{parisotto2015actor} are proposed to train a single policy by using the guidance of several expert teachers. These methods perform well on already encountered tasks or tasks with known structures. However, in most applications, robots often face unknown tasks, 
making it difficult to ensure the performance of fused control strategies in these unfamiliar scenarios.

To guarantee performance on new tasks, knowledge fusion typically requires an additional adaptation process. 
For instance, \citet{liu2021lifelong} leveraged lifelong learning techniques, specifically Gradient Episodic Memory~\cite{lopez2017gradient}, to learn a navigation policy complementary to classical motion planners to adapt to new navigation scenarios without forgetting previous ones.  \citet{liu2019lifelong} built on federated learning to efficiently acquire prior knowledge from different environments and dynamically adjust the shared model to support robots in quickly adapting to diverse navigation tasks. ~\citet{logacjov2021learning} adopted dynamic generation and adjustment of network structures to adapt prior knowledge, leveraging unsupervised knowledge integration for new task adaptation in long-term human-robot interactions with a simulated humanoid robot.
%With the development of Large Language Models (LLMs), \citet{parakh2024lifelong} used LLMs as planners that decompose high-level instructions into executable steps, enabling robots to adapt to new tasks with human assistance.
Lifelong learning is highly storage-efficient, as it retains only one model that solves all scenarios over the learning lifespan. %This also makes it susceptible to task order bias and catastrophic forgetting. Additionally, while lifelong learning 
However, as the model tries to avoid forgetting existing knowledge, it may negatively impact the efficiency of acquiring a new one due to contradicting gradients.


Meta-learning~\cite{kaushik2020fast}, on the other hand, adopts a different adaptation mechanism. It trains a meta-model which can then be adapted to many other models, one for each task.
Notable examples for metal-learning include applications in legged robots for adapting to changing dynamics~\cite{song2020rapidly} and optimization-based methods like Model-Agnostic Meta-Learning (MAML)~\cite{finn2017model}, which learns initializations that allow fast policy convergence on new tasks.
%\sout{While meta-learning enables rapid adaptation to new tasks by leveraging general prior knowledge, its adaptation heavily relies on second-order gradients, making the optimization process more complex and the convergence more challenging.}
In terms of fusing prior knowledge, meta-models typically treat all prior knowledge equally, which lacks the capability to dynamically prioritize specific prior knowledge relevant to the context of a new task.


\subsection{Context-awareness for Reinforcement Learning}
Context-aware learning considers a set of Markov Decision Processes (MDPs) that share the same state and action spaces but differ in transition probabilities and rewards based on contextual variations. Thus, a learning model can be made adaptive, by using context-awareness as an augmented input~\cite{hallak2015contextual,li2018context,lee2020context}. For example, in the work by~\citet{hallak2015contextual}, contextual MPD is proposed to model how human decision-making varies depending on their surrounding environment. Context-Aware Policy reuSe (CAPS) \cite{li2018context} leverages contexts as identifiers to determine when and which source policies should be reused.
For robotic applications, \citet{lee2020context} used a latent context vector to capture robot-specific structural features, enabling the prediction of future states.
For quadruped robot control on diverse terrains, ~\citet{kumar2021rma} treated environmental encodings as contexts, which are then used as an extra argument to a base policy for quick adaptation. %Specifically, \citet{peng2020learning} directly derived environmental encodings, while \citet{kumar2021rma} employed an additional mechanism to infer these encodings inversely from state transitions. 
For these existing works, context is typically represented as latent encodings of either environments or robots, generated during end-to-end training processes. In contrast, our work directly uses state transitions as contexts, bypassing the need for latent representations.
Moreover, while existing methods primarily rely on data-driven mechanisms to map the impact of context on model outputs, our approach explicitly integrates context to guide knowledge adaptation, which offers a more interpretable and structured way to enhance robot learning efficiency.


%Another adaptation method for robot learning is lifelong learning, which focuses on robots' continuous knowledge acquisition, adaptation, and transfer across a robot’s operational lifespan. \sout{For example, ~\cite{liu2019lifelong} proposes a lifelong federated reinforcement learning architecture that enables robots to integrate and transfer experiences/knowledge for navigation tasks. The work in~\cite{logacjov2021learning} emphasizes continuous knowledge acquisition and adaptation in long-term human-robot interactions with a simulated humanoid robot. With the development of Large Language Models (LLMs), \cite{parakh2024lifelong} uses them as planners that decompose high-level instructions into executable steps, enabling robots to adapt to new tasks with human assistance. In summary, the core of adaptation in lifelong learning lies in developing a policy that retains prior knowledge. However, this approach does not account for the impact that changes in dynamics caused by new tasks may have on the policy.}
%For example, 
%\marginXW{I don't quite understand the logic here. For the literature review, apart from what they did, answer the question: why there are `related works', and what are the limitations.}


%\marginXW{what is the lifelong learning element.}
%In summary, lifelong learning typically leverages prior knowledge by focusing on the importance of network parameters or storing critical samples or features from previous tasks. However, lifelong learning faces challenges related to the high cost of storing and managing task knowledge, making it difficult to implement in resource-constrained environments. Additionally, in the adaptation process, lifelong learning may suffer from task order bias or catastrophic forgetting, potentially overlooking earlier acquired knowledge that could be more suitable for subsequent unknown tasks.

%Lots of attempts have been proposed for the adaptation of robotics tasks. Meta-training several initial starting points for model parameters allows robots for rapid adaptation to new situations with minimal data \cite{kaushik2020fast}. The meta-learning method is also applied legged robots to quickly adapt to changes in dynamics \cite{song2020rapidly}. Meta-learning in RL aims to learn how to learn, enabling fast adaptation to new tasks. Model-agnostic meta-learning (MAML) \cite{finn2017model} is a popular optimization-based meta-learning algorithm that learns an initialization for rapid adaptation. Meta-learning primarily aims to obtain a well-initialized set of parameters that allows the policy network to converge more quickly in a new task. While this demonstrates faster adaptation to new tasks, it completely overlooks the contextual dynamics of the new task, relying solely on second-order gradients to learn a learning process for policies. Moreover, meta-learning heavily depends on policy-based reinforcement learning algorithms.

%Another general learning adaptation in robotics is lifelong learning. Lifelong learning in robotics focuses on enabling robots to continuously acquire, adapt and transfer knowledge throughout their operational lifespan. \cite{liu2019lifelong} proposes a lifelong federated reinforcement learning architecture that enables robots to fuse and transfer experiences, effectively utilizing prior knowledge for navigation tasks. \cite{logacjov2021learning} emphasizes continuous knowledge acquisition and adaptation in long-term human-robot interactions with a simulated humanoid robot. With the development of Large language Models (LLMs), \cite{parakh2024lifelong} uses it as planners that decompose high-level instructions into executable steps, enabling robots to adapt to new tasks with human assistance. In summary, the core of adaptation in lifelong learning lies in developing a policy that retains prior knowledge. However, this approach does not account for the impact that changes in dynamics caused by new tasks may have on the policy.







% RMA~\cite{kumar2021rma} enables real-time adaptation of quadruped robots to diverse and unseen terrains. RMA combines a base policy with an adaptation module that predicts latent environmental parameters, such like friction and terrain height, in real-time. 




%\cite{hallak2015contextual}, which incorporates context into decision-making.
%Context-Aware Policy reuSe (CAPS) \cite{li2018context} leverages multi-policy reuse by learning a source selection policy based on context. It dynamically identifies when and which source policy to reuse and when to terminate its reuse, but the context here is represented as a subset of states. \cite{lee2020context} introduces a context latent vector that encodes local dynamics from recent experiences. However, the model is able to predict state transitions by conditioning on this latent vector. And it only addresses the challenge of generalizing model-based RL methods to unseen environments without considering model-free RL methods. 

%Rapid Motor Adaptation (RMA)~\cite{kumar2021rma}, which inversely estimates environmental encoding from state transitions. 

%\cite{yu2017preparing}

%In robotic applications, RMA \cite{kumar2021rma} enables real-time adaptation of quadruped robots to diverse and unseen terrains. RMA combines a base policy with an adaptation module that predicts latent environmental parameters, such like friction and terrain height, in real-time. 
%\marginXW{This needs to be updated. Check page 2, second paragraph of ref RMA ~\cite{kumar2021rma} to enhance the literature here. RMA paper is a good point to start with, you can also see who cited RMA to find more related references.
%Check the revised intro, where I compared our work with RMA and other related works. To basically want to expand it here.}
%\cite{liang2023context} utilizes an attention-based policy network that reasons over the context of a robot’s belief about the known area and then filters redundant nodes in its graph representation to enhance global planning efficiency. Our CARoL realizes context-awareness by analyzing state transition in robotic task dynamics to identify similarities between the new task and all other tasks for prior knowledge.

%Difference: context is used as an input of the model; all data-driven.

%indiscriminate

%Context-aware learning has been developed after Contextual Markov Decision Processes (CMDPs) \cite{hallak2015contextual} is put forward to incorporate context into the decision-making process. After the foundation of CMDPs, Context-Aware Policy Reuse (CAPS) \cite{li2018context} leverages multi-policy reuse by learning a source selection policy based on context. It dynamically identifies when and which source policy to reuse and when to terminate its reuse, but the context here is represented as a subset of states. \cite{lee2020context} introduces a context latent vector that encodes local dynamics from recent experiences. However, the model is able to predict state transitions by conditioning on this latent vector. And it only addresses the challenge of generalizing model-based RL methods to unseen environments without considering model-free RL methods. In robotic applications, RMA \cite{kumar2021rma} enables real-time adaptation of quadruped robots to diverse and unseen terrains. RMA combines a base policy with an adaptation module that predicts latent environmental parameters, such like friction and terrain height, in real-time. 

==> Contents/method.tex <==
\section{Context-aware Adaptation for Robot Learning (CARoL)}

To explain the rationale behind CARoL, note that in a given MDP, the transition probability $\mathcal{P}_i$ plays a central role in determining the knowledge $\mathcal{K}_i$ required to solve the problem. This makes $\mathcal{P}_i$ a natural choice as the contextual marker for knowledge adaptation: greater similarities in state transitions indicate stronger relevance between the knowledge associated with a source task and that needed for a new target task.
While existing methods often rely on environmental or robot features to implicitly capture this relationship, our approach explicitly uses state transitions as the context for adaptation. This provides a more interpretable and structured method to enhance learning efficiency.

\begin{figure}
    \centering
    \includegraphics[width=0.42\textwidth]{Contents/Figures/RSS_alg_overview.pdf}
    \caption{The overview of CARoL framework. }
    \label{fig:alg_overview}
    \vspace{-1em}
\end{figure}

%In the following, w
We present details of the proposed CARoL algorithm. 
As illustrated in Fig. \ref{fig:alg_overview}, CARoL consists of three key steps. 
(i) Acquiring both the context representation and prior knowledge for each source task.
(ii) Evaluating the contextual similarities between the target task and source tasks.
(iii) Performing contextual knowledge adaptation, which can be applied to policy-based, value-based, or actor-critic RL approaches.

%First, it acquires both the context representation and prior knowledge for each source task. Second, it evaluates the contextual similarities between tasks. Finally, it performs knowledge adaptation, which can be applied to policy-based, value-based, or actor-critic reinforcement learning (RL) approaches.






%First, we provide an overview of the framework, followed by a detailed explanation of its implementation. We then discuss how the algorithm can be applied to policy-based, value-based, or actor-critic-based reinforcement learning (RL) approaches, respectively.

%As shown in Fig. \ref{fig:alg_overview}, CARoL uses three steps to adapt existing knowledge to a new target task. The challenge here is that the target task is unseen and unknown for the robot. Under these conditions, to solve such a target task using robot learning, we typically have to learn from scratch, which is extremely resource-intensive. In CARoL, we suppose to have one knowledge library which is a collection of prior knowledge. Each prior knowledge $\mathcal{K}$ represents a policy or a value function from the corresponding source task. We assume that all source tasks have different contextual dynamics, and the target task is similar to but distinct from all source tasks. CARoL has two modules to efficiently leverage prior knowledge to enhance learning the target task. 


%As shown in the Fig. \ref{fig:alg_overview}, CARoL has one target task to solve. The challenge here is that the target task is unseen and unknown for the robot. Under these conditions, to solve such a target task using robot learning, we typically have to learn from scratch, which is extremely resource-intensive. In CARoL, we suppose to have one knowledge library which is a collection of prior knowledge. Each prior knowledge $\mathcal{K}$ represents a policy or a value function from the corresponding source task. We assume that all source tasks have different contextual dynamics, and the target task is similar to but distinct from all source tasks. CARoL has two modules to efficiently leverage prior knowledge to enhance learning the target task. 


\noindent\textbf{Context Representation.}
For each source task $\mathbf{T}_i$, along with the standard use of RL that acquires the knowledge $\mathcal{K}_i$, we also train an approximation of the transition function to represent the context, denoted by $f_i(s_i,a_i~|\phi_i):\mathcal{S}\times \mathcal{A}\to \mathcal{S}$ for each source task. This function predicts the next state based on the current state-action pair and is parameterized by $\phi_i$. The parameters are updated via gradient descent for the $i$-th task:
\begin{align}
    \label{eqa:gradient}
    \phi_i' = \phi_i - \alpha \nabla_{\phi_i} \mathcal{L}_{\mathbf{T}_i}(\phi_i),
\end{align}
where $\alpha$ is the learning rate and the task collects state-action-next state triplets $\{(s_{i,k}, a_{i, k} ,s^+_{i, k})\}$ sampled from robot trajectories, with $k\in\{1,\cdots,m_i\}$ being the indicator of samples. The loss function is defined as the difference between the next true state from samples and the predicted next state:
%\begin{align}
$\mathcal{L}_{\mathbf{T}_i}(\phi_i) = \sum_{k=1}^{m_i} \|f_i(s_{i,k}, a_{i,k}~|\phi_i) - s^+_{i,k}\|^2.$
%\end{align}


\medskip
\noindent\textbf{Evaluation of Contextual Similarity.}
We use state transition functions $f_i(\cdot)$ to evaluate the contextual similarity between source task $i$ and the new target task, which quantifies the relevance of their knowledge. A straightforward approach is to learn a transition function $f_g(\cdot)$ for the new task, then compare it with $f_i(\cdot)$ from source tasks. However, learning $f_g(\cdot)$ for a new task can be computationally expensive. 

To address this, our method uses sampled trajectories $\{(s_{g,k}, a_{g, k} ,s^+_{g, k})\}$, $k\in\{1,\cdots,m_g\}$ from the target task. These samples are applied to each state transition function $f_i(\cdot)$, $i\in\{1,\cdots,n\}$ learned from the source tasks to compute their similarity, that is, for source task $i$:
\begin{align}
    \label{eqa:transition}
    \mathcal{Y}_{i} = \sum_{k=1}^{m_g}\|f_i(s_{g, k}, a_{g, k})- s^+_{g, k}\|^2.
\end{align}

A smaller value of $\mathcal{Y}_{i}$ indicates a higher contextual similarity between $i$-th source task and the target task. We regulate these measures into weights as $i\in \{1,\cdots,n\},$
\begin{align}
    \label{eqa:weight}
    w_i = \frac{\exp(-\mathcal{Y}_{i})}{\sum_{j=1}^n \exp(-\mathcal{Y}_{j})}.
\end{align}

%The first module is context-aware module. As shown in the Fig. \ref{fig:alg_overview}, we can not only obtain various prior knowledge from all the source tasks, but also learn the corresponding state transitions from them. State transitions refer to the process by which an agent moves from one state to another in a given task, based on the action it takes and the contextual dynamics. According to the Assumption \ref{assumption:context}, we use state transitions to represent the contextual information contained within the corresponding task. To obtain the transition function $\mathcal{P}_i$ for $i$-th source task, we initialize the transition function $\mathcal{P}_i$ with parameters $\phi_i$. The transition function $\mathcal{P}_i$ is used for next state prediction with the input of state-action pair under $i$-th task with $k$-th timestep, i.e., $\hat{s_{i,k+1}}=\mathcal{P}_i(s_{i, k}, a_{i,k})$. We update the parameters via gradient descent for $i$-th task:

\begin{comment}
\begin{algorithm2e}
\SetAlgoLined
\caption{Context-aware Module}
    \textbf{input} source tasks $\mathcal{T}_1, \mathcal{T}_2, \dots, \mathcal{T}_n$;\\
    \textbf{initialize} transition function approximators $\mathcal{P}_1(s,a|\phi_1), \mathcal{P}_2(s,a|\phi_2), \dots, \mathcal{P}_n(s,a|\phi_n)$ with parameters $\phi_1, \phi_2, \dots, \phi_n$;\\
    \For{each source task $\mathcal{T}_i$}{
    \For{iteration = 1 to $K$}{
        Collect a set of trajectories $\tau_i$ by random explorations;\\
            Shuffle the collected data;\\
            \For{each minibatch of data}{
            Update parameters $\phi_i$ for $\mathcal{P}_i$ with equation ~\ref{eqa:gradient};\\
            }
    }
    }
\Return{updated transition functions $\mathcal{P}_1(s,a|\phi_1), \mathcal{P}_2(s,a|\phi_2), \dots, \mathcal{P}_n(s,a|\phi_n)$.}

\end{algorithm2e}
\marginXW{distillation is a model-free method. But here, for the state transition representation, isn't it just learning the model? If not, can we justify the difference?}
\end{comment}



%context-aware module, CARoL obtains all transition functions from source tasks. We sample some exploration data, i.e., state-action-next state pairs, from the target task. Assume we have $m$ pairs, $(s_{g, 1}, a_{g, 1} ,s_{g, 2}), (s_{g, 2}, a_{g, 2} ,s_{g, 3}), \dots (s_{g, m}, a_{g, m} ,s_{g, m+1})$. We take each state-action pair as input and feed it into all the transition functions. This allows us to obtain the different predicted next states produced by the transition functions trained on various source tasks. For each transition function, we can compute the loss between the sampled state-action pair's predicted next state and the true next state from the exploration data. Let this loss for a transition function $\mathcal{P}_i$ be denoted as $\mathcal{L}_{\mathcal{S}_i}$, we have 



\noindent\textbf{Context-aware Adaption.}
The similarity weights $w_i$ enable the robot to prioritize knowledge from the corresponding source tasks. This makes its adaptation to the target task more focused and effective. 
In RL, different approaches such as policy-based, model-based, or actor-critic-based have distinct learning mechanisms. Thus, the adaption processes are also different, as we describe next.

\subsubsection{CARoL for Policy-based RL}
Suppose the knowledge $\mathcal{K}_i$ of each source task is a pre-trained policy, denoted by $\pi_i(s):\mathcal{S}\to\mathcal{A}$. 
The contextual similarity weights are $w_i$.
Let the target policy $\pi_g(s|\theta_g)$ be parameterized by $\theta_g$ and assume it interacts with the target environment on-policy to generate an action distribution $\pi_g(s|\theta_g)$ based on the current state $s \in \mathcal{S}$ and parameter $\theta_g$. Let $\xi_g$ represent the set of trajectories explored by the policy in the target task and each trajectory $\tau \in \xi_g$ is a sequence of state-action pairs.

To incorporate the knowledge from source policies $\pi_i(s)$, we define a learning loss based on the divergence between the action distribution of the target policy and a weighted combination of the action distributions of the source policies:
\begin{align}
    \label{eqa:policy_adaptation}
    \mathcal{L}_{P}=\sum_{\tau\in \xi_g} \sum_{s \in \tau}\sum_{i=1}^n w_i \mathcal{D} (\pi_i(s), \pi_g(s|\theta_g)),
\end{align}
Where $\mathcal{D}(\cdot, \cdot)$ is the Kullback–Leibler (KL) divergence: 
\begin{align}
    \label{eq:kl}
    \mathcal{D} (\pi_i(s), \pi_g(s|\theta_g)) =  \Phi(\frac{\pi_i(s)}{T}) ln \frac{\Phi(\frac{\pi_i(s)}{T})}{\Phi( \pi_g(s|\theta_g)))}.
\end{align}

Here, $\Phi(\cdot)$ is the softmax function and $T$ is the temperature parameter. 
%By minimizing the re-weighted loss $\mathcal{L}_{P}$, the parameters of the target policy $\theta_g$ are iteratively updated through gradient-based optimization. 
The process selectively incorporates knowledge from relevant source policies to optimize the target task, as summarized in Algorithm \ref{Alg_policy}.

%\vspace{-0.5em}
\begin{algorithm2e}\label{Alg_policy}\bitsmall
\SetAlgoLined
\caption{CARoL for Policy-based RL}
    \textbf{input} Knowledge as pre-trained source policies $\{\pi_1,  \dots, \pi_n\}$; contextual similarity weights $\{w_1,\cdots,w_n\}$; the target task $\mathbf{T}_g$;\\
    \textbf{initialize} target policy $\pi_g(s|\theta_g)$; a learning rate $\eta$;\\
    \For{iteration = 1 to $K$}{
        Collect trajectories $\xi_g$ by interacting with the target task $\mathbf{T}_g$ using $\pi_g(s|\theta_g)$;\\
        %Shuffle the collected data;\\
            \For{each minibatch of data from $\xi_g$}{
            Compute $\mathcal{L}_{P}$ with equation ~\eqref{eqa:policy_adaptation};\\
            Update: $\theta_g' = \theta_g - \eta \cdot \nabla_{\theta_g} \mathcal{L}_{P}$;\\
            }
    }
\Return{target policy $\pi_g$.}\
\end{algorithm2e}
%\vspace{-0.5em}


\subsubsection{CARoL for Value-based RL}
Value-based RL algorithms use value functions to estimate the expected cumulative reward starting from a given state-action pair (or from a state), then guide action selection.
In the following, we consider the knowledge $\mathcal{K}_i$ of each source task to be a pre-trained state-action value function $Q_i(s,a):\mathcal{S}\times\mathcal{A}\to\mathbb{R}$ (a similar mechanism can be easily generalized to state value function $V_i(s)$.) . 
The contextual similarity weights are $w_i$.
%Based on the weighting factor for contextual similarity, our goal is to derive a value function for the target task by fusing prior knowledge, which can effectively guide its action selection.

Let the target value function be a neural network $Q_g(s,a~|\psi_g)$ parameterized by $\psi_g$. %which estimates the value of a state-action pair for the target task. 
%Following the general approach in value-based RL algorithms, 
Actions are greedily selected for the target task using an epsilon-greedy strategy, transitioning from early exploration to later exploitation.
During exploitation, we select the action that yields the highest $Q$-value output from the current state in the $Q$-network.
%Data collected during exploration and exploitation is stored in a replay buffer for future updates.

Once the replay buffer reaches a sufficient size, we randomly extract a minibatch $\mathcal{B}$ of data. For each data pair in this minibatch, the target value is computed. However, unlike traditional value-based RL algorithms, we do not rely on the inadequately trained target $Q_g$-network for updates. Instead, we leverage the knowledge from the source $Q_i(s,a)$ functions, reweighted by contextual similarities, as follows:
\begin{align}
    \label{eqa:q_next}
    Q_{\text{next}} = \sum_{i=1}^n w_i Q_i(s^+, \arg \max\limits_{a^+} (Q_i(s^+, a^+))),
\end{align}
where $s^+$ is the next state, and $\arg\max$ selects the action by maximizing each source $Q_i$ value function.
%\marginXW{where do you use the minibatch $\mathcal{B}$?}

Using the Bellman equation with a discount factor $\gamma$, we define the following learning loss based on the difference between the target value function and the value using reweighed source $Q_i$ networks as prior knowledge:
\begin{align}
    \label{eqa:td_loss}
    \mathcal{L}_{Q}= \sum_{s \in \mathcal{B}}\left[\|Q_g(s,a~|\psi_g)-r - \gamma Q_{\text{next}}\|^2\right],
\end{align}
where $\mathcal{B}$ is the minibatch extracted from the replay buffer, and $r$ is the reward for the corresponding state-action pair.

%By minimizing the reweighed loss $\mathcal{L}_{Q}$, the parameters of the target value function, $\psi_g$, are iteratively updated by the following Algorithm \ref{Alg_value}. 
The process, summarized in Algorithm \ref{Alg_value}, selectively incorporates knowledge from the relevant source value functions to approximate the value function for the target task. To test the learned $Q_g(s,a~|\psi_g)$ in $\mathbf{T}_g$, the greedy method can be used to select actions.


\begin{algorithm2e}[h]\label{Alg_value}\bitsmall
\SetAlgoLined
\caption{CARoL for Value-based RL}
    \textbf{input} Knowledge as pre-trained source Q networks $\{Q_1, Q_2, \dots, Q_n\}$; contextual similarity weights $\{w_1,\cdots,w_n\}$; the target task $\mathbf{T}_g$;\\
    \textbf{initialize} target value function network $Q_g(s, a~|\psi_g)$; a replay buffer $\mathcal{M}$; a learning rate $\eta$\\
    \For{episode = 1 to $K$}{
    Greedy method to choose action $a$ with explorations or $\arg \max\limits_a (Q_g(s, a~|\psi_g))$ in target task $\mathbf{T}_g$ to get next state $s'$ and reward $r$;\\
    Store $(s, a, r, s')$ in $\mathcal{M}$;\\
    \If{the size of $\mathcal{M}$ is sufficient}{
    Randomly sample a minibatch $\mathcal{B}$ from $\mathcal{M}$;\\
    Compute $\mathcal{L}_{Q}$ with equation ~\eqref{eqa:td_loss};\\
    Update: $\psi_g' = \psi_g - \eta \cdot \nabla_{\psi_g} \mathcal{L}_{Q}$;\\
    }
    }
\Return{ target value function $Q_g$.}\
\end{algorithm2e}
%\vspace{-0.5em}



\subsubsection{CARoL for Actor-Critic RL}
If the prior knowledge $\mathcal{K}_i$ is in the form of an actor-critic structure, involving both a policy and a value function, then both of them can be leveraged to enhance learning in a new task.
Instead of directly combining the methods introduced earlier to simultaneously learn a policy and a value function for the target task, we focus on learning a target actor (i.e., policy) $\pi_g(s \mid \theta_g)$, while adopting a static fusion method to leverage the source critic (value) functions without using a parameterized function approximation. Otherwise, if the actor and critic are updated simultaneously, the method might suffer from issues such as instability and overestimation of $Q$-values, which are common in actor-critic RL~\cite{van2016deep}.

Similar to the policy-based approach outlined in Algorithm \ref{Alg_policy}, we define part of the learning loss to be $\mathcal{L}_P$, which measures the weighted combination of divergences between the target policy's action distribution and source action distributions.


Additionally, %recall that in actor-critic methods, the actor $\pi_g$ is trained to select an action $a = \pi_g(s)$ for a given state $s$ that maximizes the value estimated by the critic. Based on this principle, 
we define a loss from critic as follows:
\begin{align}
    \label{eqa:actor_critic_loss_2}
    \mathcal{L}_{C}=-\sum_{\tau\in \xi_g} \sum_{s \in \tau}\left[\sum_{i=1}^n w_i \cdot Q_i(s,\pi_g(s|\theta_g))\right],
\end{align}
where the action for each state $s$ is determined by the current actor $\pi_g$. Thus, $\mathcal{L}_{C}$ evaluates the performance of the target actor using the weighted combination of source critics, prioritizing those that are more contextually similar to the target task. Minimizing $\mathcal{L}_{C}$ helps to iteratively improve the target actor by leveraging the guidance of source critics. 

The combined losses in \eqref{eqa:policy_adaptation} and \eqref{eqa:actor_critic_loss_2} yields:
\begin{align}
    \label{eqa:lossAC}
    \mathcal{L}_{AC}=\mathcal{L}_{P}+\beta\mathcal{L}_{C}.
\end{align}
By minimizing $\mathcal{L}_{AC}$, the target actor $\pi_g$ is informed by both the source actors $\pi_i(s)$ through $\mathcal{L}_P$ as well as the source critics $Q_i(s,a)$ through $\mathcal{L}_C$. The value of $\beta\in\mathbb{R}_+$ is adjustable and determines the importance of each. %This process ensures that the target actor effectively integrates knowledge from both the source actors and critics to improve performance on the target task. 
Algorithm \ref{Alg_AC} summarizes how to use CARoL for actor-critic RL.  

%\vspace{-0.5em}
\begin{algorithm2e}\label{Alg_AC}\bitsmall
\SetAlgoLined
\caption{CARoL for Actor-Critic RL}
    \textbf{input} Knowledge as pre-trained source actors $\Pi = \{\pi_1, \pi_2, \dots, \pi_n\}$ and critics $\{Q_1, Q_2, \dots, Q_n\}$; contextual similarity weights $\{w_1,\cdots,w_n\}$; the target task $\mathbf{T}_g$;\\
    \textbf{initialize} target actor $\pi_g(s|\theta_g)$;\\
    \For{iteration = 1 to $K$}{
        Collect trajectories $\xi_g$ by interacting with the target task $\mathbf{T}_g$ using $\pi_g(s|\theta_g)$;\\
        %Shuffle the collected data;\\
            \For{each minibatch of data from $\xi_g$}{
            Compute $\mathcal{L}_{AC}$ with equation ~\eqref{eqa:policy_adaptation} and \eqref{eqa:actor_critic_loss_2};\\
            Update: $\theta_g' = \theta_g - \eta \cdot \nabla_{\theta_g} \mathcal{L}_{AC}$;\\
            }
    }
\Return{target actor $\pi_g$.}\
\end{algorithm2e}




\subsubsection{CARL+}\label{sec_Carol+}
In the above subsections, the introduced CARoL focuses on leveraging prior knowledge to solve a new target task. It omits the aspect of using standard RL approaches to acquire new knowledge from the task. This is because additional learning may not always be necessary when prior knowledge is already sufficient for solving the task.
However, if learning from the target task is required, this can be achieved by adding standard RL loss terms to the functions \eqref{eqa:policy_adaptation}, \eqref{eqa:td_loss}, and \eqref{eqa:lossAC} for policy-based, value-based, and actor-critic methods, respectively. This straightforward extension enables the model to not only adapt prior knowledge but also refine it through direct learning from the target task. An implementation of this, called CARoL+, will be included in the experiments section for comparison.


\begin{comment}
\begin{algorithm2e}
\SetAlgoLined
\caption{Similarity Module}
    \textbf{input} updated transition functions $\mathcal{P}_1(s,a|\phi_1), \mathcal{P}_2(s,a|\phi_2), \dots, \mathcal{P}_n(s,a|\phi_n)$;\\
    \textbf{input} target task $\mathcal{T}_g$;\\
    \For{iteration = 1 to $K$}{
        Collect a set of trajectories $\tau_g$ by random explorations;\\
            \For{each transition functions $\mathcal{P}_i$}{
            Compute the loss $\mathcal{L}_{\mathcal{S}_i}$ with equation ~\ref{eqa:transition};
            }
        Compute the similarity weight set $\mathbf{W}$ with equation ~\ref{eqa:weight} for each source task;\\
    }
    Compute the average similarity weight set $\mathbf{W}$:
    $\mathbf{W} = \frac{1}{K} \sum_{iteration=1}^{K} \mathbf{W}^{(iteration)}$;\\
\Return{the similarity weight set $\mathbf{W}$.}\
\end{algorithm2e}
\end{comment}
%The similarity weights enable the robot to prioritize the knowledge for each teacher knowledge corresponding to its source task. The higher weight indicates that the target task and the corresponding source task share highly similar contextual dynamics. This better guides the robot's learning direction of prior knowledge, making its adaptation to the target task more focused and effective. In RL, since we distinguish between policy and value function as forms of knowledge, our adaptation is also differentiated based on these two types of knowledge.




%The parameters of the target policy, $\theta_g$, are updated by minimizing the adaptation loss $\mathcal{L}_{P}$ via gradient-based optimization:
%\begin{align}
%    \label{eqa:policy_update}
%    \theta_g' = \theta_g - \eta \cdot \nabla_{\theta_g} \mathcal{L}_{P}
%\end{align}
%The above steps are repeated iteratively, where the target policy selectively incorporates the knowledge from source policies for solving the target task.



%The goal is to efficiently obtain a policy $\pi_g(s|\theta_g)$ for the target task.

%To enable efficient policy adaptation in the target task, CARoL initializes a student policy and iteratively refine based on the student policy's exploration in the target task. The adaptation is guided by leveraging multiple pre-trained teacher policies from source tasks, weighted by their similarity to the target task. This process ensures the student policy effectively incorporates prior knowledge while being tailored to the target task.

%The student policy, denoted as $\pi_s(a|s;\theta_s)$ is initialized with parameters $\theta_s$. The policy is responsible for generating actions in the target task environment. At each iteration, the student policy interacts with the target environment, exploring states $s \in \mathcal{S}_g$. For each state $s$, the student policy generates an action distribution $\pi_s(a|s)$. Assume a set of pre-trained teacher policies $\{\pi_i(a|s;\theta_i)\}^n_{i=1}$ is available, each trained on a source task. Assume the similarity weights $\{w_i\}^n_{i=1}$ is computed from similarity module, representing the relevance of each teacher policy. For each explored state $s$, the adaptation loss is computed based on the divergence between the student policy’s action distribution and a weighted combination of the teacher policies’ action distributions.
%\begin{align}
%    \label{eqa:policy_adaptation}
%    \mathcal{L}_{\text{adapt}}=\sum_{s\in \tau_g} \sum_{i=1}^n w_i \mathcal{D} (\pi_i(s), \pi_s(a|s))
%\end{align}
%Where $\tau_g$ represents the set of trajectories explored by the student policy in the target task. $\mathcal{D}(\cdot, \cdot)$ here is the Kullback–Leibler (KL) divergence: 
%\begin{align}
%    \label{eq:kl}
%    \mathcal{D}_{KL} =  \Phi(\frac{\pi_i(s)}{T}) ln \frac{\Phi(\frac{\pi_i(s)}{T})}{\Phi( \pi_s(a|s)))} 
%\end{align}
%where $\Phi(\cdot)$ is the softmax function and $T$ is the KL temperature. The parameters of the student policy, $\theta_s$, are updated by minimizing the adaptation loss $\mathcal{L}_{\text{adapt}}$ 
%via gradient-based optimization:
%\begin{align}
%    \label{eqa:policy_update}
%    \theta_s' = \theta_s - \eta \cdot \nabla_{\theta_s} \mathcal{L}_{\text{adapt}}
%\end{align}
%The above steps are repeated iteratively. With each update, the student policy incorporates more refined knowledge from the teachers while improving its performance in the target task.


%Therefore, the value function also serves as a critical source of prior knowledge that can be obtained from source tasks. Typically, value functions are categorized into state value functions and action value functions. In our subsequent work, we focus on the action value function, as it directly evaluates the value of state-action pairs. This property makes it particularly effective for guiding action selection and robot control in new tasks, enabling rapid adaptation through the utilization of prior knowledge.




%The value function is a fundamental component of RL that estimates the expected cumulative reward starting from a given state (or state-action pair). Therefore, the value function also serves as a critical source of prior knowledge that can be obtained from source tasks. Typically, value functions are categorized into state value functions and action value functions. In our subsequent work, we focus on the action value function, as it directly evaluates the value of state-action pairs. This property makes it particularly effective for guiding action selection and robot control in new tasks, enabling rapid adaptation through the utilization of prior knowledge.

%Similar to policy adaptation, in adaptation for value function, we assume that each source task has a pre-trained critic $\mathcal{Q} = \{Q_1, Q_2, \dots, Q_n\}$, where each teacher critic provides value estimates for state-action pairs in its respective source task. 
% While the target task is unseen and distinct, we assume it is similar to the source tasks, sharing the same state space and action space as all source tasks.

%We first initialize a student Q-network and a replay buffer. Following the general approach of RL algorithms, we start by greedily choosing actions on the target task, for instance, using an epsilon-greedy strategy, transitioning from early exploration to later exploitation. Here, since we use value-based adaptation, our exploitation involves selecting the action that yields the highest Q-value output from the current state in the Q-network. During this ongoing process of exploration and exploitation, the data collected is stored in the replay buffer initialized at the beginning.

%When the replay buffer size becomes sufficient, we randomly extract a minibatch of data from it. For each pair in this minibatch, we compute the target value. However, unlike traditional value-based RL algorithms, our value adaptation does not utilize a target Q-network. Instead, when calculating $Q_{\text{next}}$, we rely on all the teacher Q-networks learned from the source tasks and incorporate the corresponding similarity weights of each teacher, rather than using a target Q-network.
%\begin{align}
%    \label{eqa:q_next}
%    Q_{\text{next}} = \sum_{i=1}^n w_i Q_i(s', \arg \max (Q_i(s', \cdot)))
%\end{align}
%The target value is still computed using the Bellman equation. Assume the discount factor is denoted as $\gamma$.
%\begin{align}
 %   \label{eqa:target_value}
 %   y = r + \gamma \times Q_{\text{next}}
%\end{align}
%And our adaptation loss is based on the divergence between the Q value from student Q nextwork and the target value weightedly evaluated from all prior knowledge.
%\begin{align}
%    \label{eqa:td_loss}
%    \mathcal{L}_{\text{adapt}}= \mathcal{D}(Q_s(s, a), y)
%\end{align}
%where we use mean square error for current $\mathcal{D}(\cdot, \cdot)$ here.

%Another objective in actor-critic adaptation is to train an actor $\pi_s$ such that, for a given state $s$, the chosen action $a=\pi_s(s)$ maximizes the value estimated by the Critic. Since our teacher critics provide a more reliable reference target by offering conservative estimates for each source task, we directly use the teacher critics combined with similarity weights to evaluate the student actor's performance for the given state $s$.

%This weighting introduces a bias, emphasizing the evaluations of teacher critics that are more contextually similar to the target task, as their assessments of state-action pairs are likely to be more relevant or accurate.
%Using this weighted critic value, we define the second part of actor-critic adaptation loss.

%By minimizing the sum of the two parts of the adaptation loss, we optimize the parameters of the student actor to enable effective adaptation to the target task.

%The overall loss is by combining \eqref{eqa:policy_adaptation} and \eqref{eqa:actor_critic_loss_2}:
%\begin{align}
%    \label{eqa:lossAC}
%    \mathcal{L}_{AC}=\mathcal{L}_{P}+\mathcal{L}_{C}
%\end{align}

%we must fully utilize all the prior knowledge during adaptation with CARoL, without discarding any part of it. For the adaptation of an actor-critic structure, we primarily integrate the processes of policy adaptation and value adaptation.

%In actor-critic adaptation, we utilize both well pre-trained teacher actors as prior knowledge and teacher critics that have been stably optimized from source tasks. It is worth noting that, unlike value adaptation, where the Q-network updates also aim to stabilize the adaptation process, the teacher critics used here are obtained after addressing the overestimation issue of Q-values, such as by employing techniques like twin critics.

%In our actor-critic adaptation algorithm, we also adopt offline data sampling as an example. However, since we initialize the student actor, we interact with the environment by combining the student actor's actions with some random perturbation to incorporate exploration. After randomly sampling from the replay buffer, we first use all the teacher actors to generate their actions for the current state. These actions are then compared with the action from the current student actor, and their similarity weights are used to perform a distance measurement, yielding the loss term 

%\begin{align}
%    \label{eqa:actor_critic_loss_1}
%    \mathcal{L}^1_{\text{adapt}}=\sum_{s\in \xi_g} \sum_{i=1}^n w_i \mathcal{D} (\pi_i(s), \pi_s(a|s))
%\end{align}

%Unlike the policy adaptation above, which requires actions to be stochastic, this adaptation approach can also handle deterministic actions. If the actions are stochastic, the distance metric $\mathcal{D}(\cdot, \cdot)$ in $\mathcal{L}_{\text{adapt}}^1$ is computed using KL divergence. If the actions are deterministic, $\mathcal{D}(\cdot, \cdot)$ is computed using MSE.

% After initializing the student actor $\pi_s$, we leverage all teacher critics to evaluate each state-action pair generated during the interaction between the student actor and the target task. With the similarity weights obtained from the similarity module, we compute a weighted Q-value for the student $Q_s(s,a)$ in the target task. 

%Another objective in actor-critic adaptation is to train an actor $\pi_s$ such that, for a given state $s$, the chosen action $a=\pi_s(s)$ maximizes the value estimated by the Critic. Since our teacher critics provide a more reliable reference target by offering conservative estimates for each source task, we directly use the teacher critics combined with similarity weights to evaluate the student actor's performance for the given state $s$.
%\begin{align}
%    Q_s(s,a) = \sum_{i=1}^n w_i \cdot Q_i(s,\pi_s(a|s))
%\end{align}
%This weighting introduces a bias, emphasizing the evaluations of teacher critics that are more contextually similar to the target task, as their assessments of state-action pairs are likely to be more relevant or accurate.

%Using this weighted critic value, we define the second part of actor-critic adaptation loss. 
%\begin{align}
%    \label{eqa:actor_critic_loss_2}
%    \mathcal{L}^2_{\text{adapt}}=-\mathbb{E}_{s \in \mathcal{B}}[Q_s(s, a)]
%\end{align}
%By minimizing the sum of the two parts of the adaptation loss, we optimize the parameters of the student actor to enable effective adaptation to the target task.





==> Contents/problem.tex <==
\section{Preliminaries and Problem Formulation} \label{sec:problem}
%We introduce the fundamentals of Markov Decision Processes (MDPs) and define the concept of \textit{knowledge} for solving an MDP. Building on these, we formulate the problem of context-aware adaptation, which seeks to enable robots to efficiently learn new tasks by leveraging prior knowledge.


\subsection{Markov Decision Processes and Knowledge} 
An RL task can be modeled by a Markov Decision Process defined as a tuple $\mathbf{T}=\{\mathcal{S},\mathcal{A}, \mathcal{P},\mathcal{R}\}$, where each element represents state space, action space, transition probability measure, and reward function, respectively. 
The objective of an RL agent is to learn a decision-making strategy that selects actions from the action space $\mathcal{A}$ based on current states in state space $\mathcal{S}$, in order to maximize the cumulative reward $\mathcal{R}$.
In this paper, we use a general notation $\mathcal{K}$ to represent the critical knowledge required for such decision-making. Depending on the RL methods employed, $\mathcal{K}$ can take various forms: For policy-based RL, it represents a policy that directly maps states to actions. For value-based RL, it represents the value function that estimates the cost-to-go which informs the choice of action; For actor-critic RL, it combines both the policy (actor) and value function (critic) ~\cite{arulkumaran2017deep}. 


\subsection{Problem Formulation}
%This paper concerns the efficient adaptation to a new task by leveraging prior knowledge from previously solved tasks.  
Consider a set of $n$ source tasks, denoted as $\mathbb{T} = \{\mathbf{T}_1, \mathbf{T}_2, \dots, \mathbf{T}_n\}$, where each source task $\mathbf{T}_i = \{\mathcal{S}, \mathcal{A}, \mathcal{P}_i, \mathcal{R}\}$ for $i \in \{1, \dots, n\}$ is defined by shared state and action spaces ($\mathcal{S}$, $\mathcal{A}$) and a common reward function ($\mathcal{R}$), but distinct transition probability measures ($\mathcal{P}_i$).
A new unseen target task is represented as $\mathbf{T}_g=\{\mathcal{S},\mathcal{A}, \mathcal{P}_g,\mathcal{R}\}$.
The target task shares the same state space, action space, and reward function as the source tasks, but its transition probability measure $\mathcal{P}_g$ is unknown.

The formulation applies to scenarios with similar objectives, such as robot navigation tasks with a consistent success metric. We can use the same state and action spaces for all scenarios, but variations in robot configurations (e.g., chassis, wheels, tires, etc.) and deployment across various terrain (e.g., geometry, surface material, etc.) will lead to differences in transition probability measures.

We assume the source tasks can be sufficiently trained to acquire a knowledge set $\mathbb{K}=\{\mathcal{K}_1,\mathcal{K}_2,\cdots,\mathcal{K}_n\}$. The problem of interest is to develop an efficient algorithm that derives the knowledge $\mathcal{K}_g$ for the target task $\mathbf{T}_g$, by leveraging the prior knowledge $\mathbb{K}$ to accelerate learning and improve performance.

%our method utilizes state transitions as the contextual representation of a task. Then, 

%two preliminaries: Contextual Markov Decision Processes and Knowledge Adaptation. Our proposed algorithm builds upon these two foundations by incorporating state transitions as a form of prior knowledge to represent task contexts. Throughout the preceding preliminaries, we formulate the problem of robot learning in a similar but distinct task.

%It is also the 

%The key issue in this problem is the lack of information about the context distributions for the source tasks and the target task. Since different contexts in a CMDP correspond to different MDP dynamics, we cannot allow the student model to blindly learn the teacher knowledge across different contexts without consideration.


%Our adaptation problem is defined as follow. Given a source task set $\mathbb{T} = \{\mathcal{T}_1, \mathcal{T}_2, \dots, \mathcal{T}_n\}$ and the target new task $\mathcal{T_g}$. All source tasks are well pre-trained, resulting in a prior knowledge library $\mathbb{K} = \{\mathcal{K}_1, \mathcal{K}_2, \dots, \mathcal{K}_n\}$, where $\forall \mathcal{K}_i \in \mathbb{K}$ denotes the teacher knowledge for corresponding source task.
%Our goal is to optimally utilize the prior knowledge from source tasks to train a student model that performs well on the unseen target task $\mathcal{T}_g$. In our problem, we assume that the contexts in all source tasks are different, while the contexts in the target task are similar but distinct from those in the source tasks. Additionally, the contexts in the target task are unknown beforehand. In this work, we also assume that each all tasks share the same state-action space. 

%Each task is a Markov Decision Process~\cite{} defined as a tuple $T_i=\{\mathcal{S},\mathcal{A}, \mathcal{P}_i,\mathcal{R}\}$
%Define the solution of the MDP.
%Direct observation is that whether knowledge can be adapted to the new environment depends on the similarity of $\mathcal{P}_i$

%All tasks share the same objectives.
%State traditions are different.

%In CMDPs, the environment dynamics and reward structure can vary depending on an underlying context. Typically, a CMDP is defined by a tuple $\{\mathcal{S},\mathcal{A}, \mathcal{P},\mathcal{R}, \mathcal{C}\}$, where the first four elements are state space, action space, transition probability measure, and reward function, respectively. The additional element $\mathcal{C}$ can be seen as representing different scenarios, conditions, or external factors, which are not directly controllable by the agent. For example, in a robot motion planning task, the context could represent different types of terrains, such as smooth floors or rough surfaces, affecting robot's movement dynamics. These environmental features influence how actions affect state transitions and the rewards obtained.
% \footnote{For an ease of presentation, we assume context only affects the transition kernel rather than reward functions. In RL, transition kernel is more important than reward function as it dictates the system dynamics. The extension to the setting where context affects reward functions can be similarly investigated.}  

%\marginXW{Is CMDP a `problem formulation', why it has a goal, and the goal is to find a policy? Are CMDPs such narrowly defined?}
%\begin{assumption}
 %   For an ease of presentation, we assume that the context only affects the state transition function rather than the reward function. In a CMDP, the impact of context on state transition primarily lies in how different contexts correspond to distinct environmental dynamics, causing the same action $a \in \mathcal{A}$ to produce different outcomes. On the other hand, the influence of context on the reward function is mainly reflected in variations in task objectives. In our work, we assume the new target task is similar but distinct, meaning that the task objectives are similar, but the environmental dynamics differ. Additionally, the extension to the setting where context affects reward functions can be similarly investigated.
%\end{assumption}

%\begin{remark}
    %\label{}
%    Based on the foundation of CMDP, the state transition function depends on the context, i.e., $P(s'|s, a; c)$ . We assume that in CMDP tasks, the dynamic contexts of a task and the state transition function form a bijective relationship. In other words, the state transition can be used to represent the contexts of a task, and different state transitions correspond to distinct contexts.
%\end{remark}

% The goal of a CMDP is to find an optimal policy that maximizes the cumulative return across all contexts in the desired task. 
% \begin{align}
%     \pi^* = \arg\max_{\pi} \mathbb{E}_{c \sim p(c)} \left[ \mathbb{E}_{s \sim \mathcal{S}} \left[ \sum_{t=0}^{\infty} \gamma^t R(s_t, a_t, c_t) \right] \right]
% \end{align}
% where $p(c)$ is the distribution of the context $c \in \mathcal{C}$. However, in many robotic scenarios, the distribution of the context in the desired task is unknown. 

%\marginXW{This paragraph does not match the fact that we use state transition as the context. You mentioned environmental features, but we explicitly stated that using environmental-context is traditional, which is worse than what we propose here.}


%\subsection{Knowledge Adaptation}
%\textcolor{blue}{
%Knowledge adaptation (KA) is a method of extracting knowledge from multiple source domains or tasks and transferring it to a target domain or task. Unlike traditional knowledge distillation, which focuses on compressing a model, knowledge adaptation emphasizes applications in domain adaptation, aiming to enable student models to learn and generalize effectively even with limited labeled data in the target domain. In RL, consider teacher knowledge $\mathcal{K}_i$ was trained on its corresponding source tasks $\mathcal{T}_i$. In the target domain $\mathcal{T}_g$, we only have access to a few exploration without any knowledge from it. The objective for KA is now to train a student model that performs well on unseen examples from the target domain.
%}

%\marginXW{The section of Knowledge Adaptation. If it's not useful and difficult to write, why not just remove it?}

% and a student policy $\hat{\pi}$, PD is formulated to minimize the difference between $\hat{\pi}(s)$ and $\pi_i(s)$ where $\pi_i \in \Pi$. Let $\theta_i$ parameter $i$-th teacher policy and $\hat{\theta}$ parameter student policy. The objective for PD is to train a student policy that closely imitates the behavior of all teacher policies as follows:
% \begin{align}
%     \label{eq:distill_loss}
%     \min_{\hat{\theta}} \mathcal{L}(\hat{\theta}) = \min_{\hat{\theta}} \mathbb{E}_{s \sim \mathcal{S}} \left[ \sum_{i=1}^n w_i \mathcal{D}(\pi_i(s), \hat{\pi}(s)) \right]
% \end{align}
% where $w_i$ represents the distillation weight for $i$-th teacher. Typically, when faced with an unseen task, PD assumes equal importance for each teacher to ensure that the robot functions adequately in the target task. However, this approach fails to capture the distinct characteristics arising from differences in contextual dynamics among prior knowledge, potentially introducing noise and diminishing the effectiveness of distillation. $\mathcal{D}(\cdot, \cdot)$ is a distance measurement between two policies. There are multiple choices for the distance metrics, such as mean square error, Kullback–Leibler (KL) divergence or cross entropy.  

% In our work, for policy-based XXX, we use KL divergence,
% \begin{align}
%     \label{eq:kl}
%     \mathcal{D}_{KL}(\hat{\theta}) =  \Phi(\frac{\pi_i(s)}{\tau}) ln \frac{\Phi(\frac{\pi_i(s)}{\tau})}{\Phi( \hat{\pi}(s))} 
% \end{align}
% where $\Phi(\cdot)$ is the softmax function and $\tau$ is the KL temperature. 

% PD cannot guarantee the performance of teacher policies in a new, unknown environment. Consequently, the student policy also loses its ability to effectively mimic the teacher policies.



% Let tasks be episodic with maximum number of steps $T$ in each episode and take acerage reward of $k$ episodes. The metric of a learning algorithm is 
% \begin{align}
%     W(k) = \frac{1}{k}\sum_{i=0}^{k}\sum_{t=0}^{T}\gamma^h R_k(s_t, a_t, c_t)
% \end{align}
% Where $R_k(s_t, a_t, c_t)$ is the reward of time step $t$ in episode $i$. The convergence speed and value of $W(k)$ indicate the learning performance.

% Our problem is defined as follow. Let $\mathcal{C}$ denote a context space and we have a source task set $\mathbb{T} = \{\mathcal{T}_1, \mathcal{T}_2, \dots, \mathcal{T}_n\}$ where the distribution of contexts, i.e., $p_i(c)$ where $c \in \mathcal{C}$, in each task $\mathcal{T}_i$ is different. Assume that each source task has well trained a teacher policy, $\Pi = \{\pi_1, \pi_2, \dots, \pi_n\}$ denotes the set of teacher policies corresponding to source tasks. The problem is that once we encounter a new, unseen and unknown target task $\mathcal{T}_g$, how we can get the optimal policy efficiently. Assume $\mathcal{T}_g$ also contains a distribution of contexts, i.e., $p_g(c)$ where $c \in \mathcal{C}$. 
% \begin{align}
%     \hat{\pi}^* = \arg\max_{\hat{\pi}} \mathbb{E}_{c_g \sim p_g(c)} \left[ \mathbb{E}_{s \sim \mathcal{S}} \left[ \sum_{t=0}^{\infty} \gamma^t R(s_t, a_t, c_t) \right] \right]
% \end{align}

% % The key is to quickly learn the optimal policy by exploiting knowledge from teacher policies. 
% By leveraging knowledge from teacher policies through policy distillation, specifically, the student policy $\hat{\pi}$ should generalize well to the target task by effectively distilling useful information from the teacher policies. The objective can be formulated as: 
% \begin{align}
%     \hat{\pi}^* = \arg\min_{\hat{\pi}}  \mathbb{E}_{c_g \sim p_g(c)} \left[ \mathbb{E}_{s \sim \mathcal{S}} \left[ \sum_{i=1}^n \mathcal{D}\left(\hat{\pi}(s|c_g), \pi_i(s|c_i)\right) \right] \right]
% \end{align}




==> Contents/results.tex <==
\section{Experiments}
In this section, we present both simulated and physical experiments to evaluate the effectiveness of CARoL in leveraging prior knowledge and context awareness to solve new tasks.

To ensure reproducibility, the simulated experiments are conducted using OpenAI's CarRacing and LunarLander tasks, as shown in Fig.~\ref{fig:sim_intro}-(a,b).
To demonstrate CARoL's capabilities in real-world scenarios (Fig. ~\ref{fig:sim_intro}-(c)), we deploy it on a ground vehicle, enabling the rapid and efficient adaptation of policies learned from source tasks to smoothly navigate real-world off-road terrain.
In these setups, CARoL is integrated with various RL algorithms for knowledge adaptation, and its performance is compared against multiple baseline approaches.
Details of algorithm implementations (CARoL and Baselines) and source code will be publicly available on GitHub.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.35\textwidth]{Contents/Figures/simulation_intro.pdf}
    \caption{Two OpenAI simulation environments for validating our algorithm: (a) CarRacing environment; (b) LunarLander environment. One physical experiment environment: (c) Ground vehicle off-road navigation.}
    \label{fig:sim_intro}
    \vspace{-1em}
\end{figure}
% \marginXW{Looks ugly. Add the real-world one.}

%For reproducibility, our simulated experiments employ the OpenAI's CarRacing and LunarLander tasks. 
%To showcase the capability of CARoL in real-world scenarios, we test on a ground vehicle to quickly and efficiently adapt policies learned in source tasks to smoothly traverse real-world off-road terrain. 

%     \item Does CARoL adapt a superior policy that handles the new physical off-road navigation task?
%For reproducibility, our simulated experiments employ the OpenAI's CarRacing and LunarLander tasks. 

%, including PPO (Proximal policy optimization)~\cite{} and TD3 (Twin Delayed Deep Deterministic)\cite{},
 
 
% we conduct our primary simulation experiments on OpenAI's CarRacing and LunarLander tasks to validate our method and compare it with baseline approaches. In these simulation experiments, we trained the teacher knowledge with the policy-oriented PPO on CarRacing and the value-oriented TD3 on LunarLander, both of which are actor-critic architectures, to demonstrate the general capability of CARoL to adapt to new tasks using prior knowledge obtained from different types. Furthermore, to showcase the potential of CARoL in real-world scenarios, we design diverse terrains in a simulation platform and adapt the learned policies to enable smooth traversal across real-world off-road terrains.
\subsection{Simulated Experiment: CarRacing}
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.85\textwidth]{Contents/Figures/reward_carracing_v2.pdf}
    \caption{Comparison of cumulative reward for CARoL and baselines under different CarRacing tasks. The x-axis represents the running steps and the y-axis represents the reward. The height of dash lines demonstrates the average accumulative reward of source knowledge (SK) under the task.}
    \vspace{-1em}
    \label{fig:carracing_reward}
\end{figure*}
\subsubsection{Experiment Setup}
As shown in Fig. \ref{fig:sim_intro}-(a), CarRacing is a continuous control task where an autonomous mobile robot must navigate a procedurally generated racetrack to maximize cumulative rewards. The task involves balancing speed and control to avoid going off-track while efficiently moving forward on the racetrack. The dynamics of the car depend on track friction. We design three different task environments with low $\mu=0.5$, medium $\mu=1$, and high friction $\mu=2$, as source tasks. To implement CARoL, 
we obtain all source knowledge (SK) using PPO (Proximal policy optimization)~\cite{schulman2017proximal}. While PPO has a value function that is used to improve training stability, it is primarily an actor-focused method. The source knowledge is represented as pre-trained source policies. Therefore, our CARoL framework utilizes Algorithm \ref{Alg_policy} for adaptation to the target tasks. 

Implementation of Baselines:
\begin{itemize} [leftmargin=*]

    \item \textbf{Policy Distillation (PD)} \cite{rusu2015policy}:  
    PD is implemented using source policies as teachers to train a target policy, which fuses all source policies equally in an indiscriminate manner.
    

    \item \textbf{Model-Agnostic Meta-Learning (MAML)} \cite{finn2017model}: We include MAML as a representative method for meta-learning. The meta-model is trained using all source tasks. Then the meta-model is adapted to the new environment using PPO.
    

    \item \textbf{Learning from Scratch (LfS)}: The same method that is used in source knowledge training but adjust the network structure to match that of CARoL.


    \item \textbf{Source Knowledge (SK)}: We directly apply source knowledge to different target tasks. The accumulative reward values are evaluated by averaging over 20 episodes.
\end{itemize} 


\begin{comment}
\begin{itemize} [leftmargin=*]
\item The observation space of the task includes four $96\times 96 \times 3$ RGB images of the top-down view of the car and track (including the current and past three time-steps), as well as the speed and gyroscope readings of the car.

\item The continuous action space consists of three dimensions: steering $[-1, 1]$, acceleration $[0,1]$, and brake $[0,1]$. 

\item The robot receives a reward for visiting new segments of the track and is penalized for each timestep. The episode terminates when the car completes the track or it goes off-track. 
% \marginXW{check if the rewordings are correct.}
\end{itemize}
In CarRacing, the dynamics of the car depend on track friction. We design three different task environments with low $\mu=0.5$, medium $\mu=1$, and high friction $\mu=2$, as source tasks. Our goal is to quickly obtain a policy in a target task with a new friction level. The friction levels for both source and target tasks are unknown to the robot.


\smallskip
\subsubsection{Implementation of CARoL and other Baselines}

\begin{itemize} [leftmargin=*]
    \item \textbf{CARoL}: In CarRacing, we obtain all source knowledge using PPO (Proximal policy optimization)~\cite{schulman2017proximal}. While PPO has a value function that is used to improve training stability, it is primarily an actor-focused method. The source knowledge is represented as pre-trained source policies. Therefore, our CARoL framework utilizes Algorithm \ref{Alg_policy} for adaptation to the target tasks. 
    
    
    
    %In CarRacing, we obtained all source knowledge using PPO (Proximal policy optimization)~\cite{schulman2017proximal}. Consequently, the source knowledge is primarily represented in the form of pre-trained source policies. Although PPO is an actor-critic method, it is heavily oriented towards the policy (actor). Therefore, our CARoL also utilizes Algorithm \ref{Alg_policy} for adaptation on the target tasks.
    % First introduce that the knowledge is obtained using PPO (Proximal policy optimization)~\cite{schulman2017proximal}. Although PPO is an actor-critic method, it is heavily oriented towards policy (actor). 
    % What is the knowledge? -> We use Alg 1...

    \item \textbf{Policy Distillation (PD)} \cite{rusu2015policy}: We include PD as a representative method for multi-task reinforcement learning in our baseline. PD is implemented using well-trained source policies as teachers to train a target policy. The key distinction between PD and CARoL lies in their adaptation mechanisms: CARoL leverages similarity weights to enable context-aware adaptation, whereas PD fuses all source policies equally in an indiscriminate manner. 
    
    %teacher policy and a student policy. Specifically, the teacher policies are identical to the source knowledge used in CARoL, having been well pre-trained using PPO. The student policy shares the same neural network structure as CARoL's target actor. The key distinction between PD and CARoL lies in the adaptation mechanism: while CARoL leverages a similarity module to facilitate adaptation, PD simply averages and fuses all teacher policies without additional adaptation.

    \item \textbf{Model-Agnostic Meta-Learning (MAML)} \cite{finn2017model}: We include MAML as a representative method for meta-learning in our baseline. The meta-model is trained using all source tasks. Then the meta-model is adapted to the new environment using PPO.
    
    %MAML is meta-trained using all source tasks. Then, we adopt the same method that is used in source knowledge training as the optimization strategy to keep the consistency. MAML optimize the initialization parameters $\theta_g$ and We demonstrate the adaptation process of the learned initialization on target tasks after meta-training.  

    \item \textbf{Learning from Scratch (LfS)}: We incorporate the same method that is used in source knowledge training but adjust the network structure to match that of CARoL, enabling learning from scratch for the target task.


    \item \textbf{Source Knowledge (SK)}: We directly apply source knowledge to different target tasks. The accumulative reward values are evaluated by averaging over 20 episodes.
\end{itemize} 

\textbf{Implementation Details}: 
    For training SKs, we employ a CNN-based actor network, consisting of 6 convolutional layers with increasing channels \{8, 16, 32, 64, 128, 256\}
    and a fully connected layer (100 units). The input of the actor-network is obtained by: first converting the (top-down view) RGB image to a grayscale image, then stacking the current image together with the images of the three previous timesteps. 
    To enable context awareness of CARoL, we learn the state transition function using a 4-layer MLP 
    \{16, 32, 16, 2\}
    with ReLU activations in the hidden layers. This model considers vehicle speed and gyroscope readings as states and steering, acceleration, and braking as actions. 
    CARoL, PD, and LfS each output a policy for the target task with the same architecture: a lighter actor network with 4 convolutional layers 
    \{8, 16, 32, 64\}
    and a fully connected layer (50 units). All models are trained using the Adam optimizer with a fixed learning rate of $1\times 10^{-4}$ and a discount factor of 0.99. The total training timesteps for SK and the inner-loop of source tasks in MAML are set to $6\times 10^6$ timesteps, while the adaptation phase for CARoL, PD, and LfS is limited to $2\times 10^6$ timesteps for faster adaptation and fair comparison. For MAML, we train the meta-policy with a meta-batch size of 3 source tasks, and the adaptation is performed over 5 gradient steps with the same learning rate.
\end{comment}

%\setlength{\tabcolsep}{5pt}

\begin{comment}
\begin{table}[]
    \caption{Contextual similarities - CarRacing.}
    \label{tab:carracing_weights}
    \centering
    \begin{tabular}{l|ccc}
    \toprule
    & $\mathbf{T}_1$ & $\mathbf{T}_2$ & $\mathbf{T}_3$ \\
    \midrule 
       \text{a: }$\mathbf{\mu=0.2}$  & 1.00 & 0.00 & 0.00 \\
       \midrule 
       \text{b: }$\mathbf{\mu=0.5}$  & 0.98 & 0.02 & 0.00 \\
       \midrule 
       \text{c: }$\mathbf{\mu=0.7}$  & 0.83 & 0.17 & 0.00 \\
       \midrule 
       \text{d: }$\mathbf{\mu=1.0}$   & 0.05 & 0.94 & 0.01 \\
       \midrule 
       \text{e: }$\mathbf{\mu=1.3}$   & 0.10 & 0.64 & 0.26 \\
       \midrule 
       \text{f: }$\mathbf{\mu=1.7}$  & 0.06 & 0.15 & 0.79 \\
       \midrule 
       \text{g: }$\mathbf{\mu=2.0}$   & 0.06 & 0.11 & 0.83 \\
       \midrule 
       \text{h: }$\mathbf{\mu=2.3}$   & 0.08 & 0.13 & 0.79 \\
       \bottomrule
    \end{tabular}
\end{table}
\end{comment}

\smallskip
\subsubsection{Results and Analysis}

Table \ref{tab:carracing_weights} presents the contextual similarity weights learned for the three source tasks in different target tasks under the CarRacing simulated experiment. We observe that the contextual similarity weight assigned to a source task for a given target task is generally negatively correlated with their friction difference. %In other words, the friction of source tasks closer to the target task tends to receive higher similarity weights, and vice versa. 
In particular, the tasks with $\mu=0.5$, $\mu=1$, and $\mu=2$ correspond to scenarios where the target task is the same as one of the source tasks. %These serve as a sanity check for the algorithm's ability to correctly identify contextual similarity. 
The results confirm the effectiveness of our approach, as the corresponding source task consistently receives the highest similarity weight.

Fig.~\ref{fig:carracing_reward} presents the reward curves, where the x-axis represents the number of training steps, and the y-axis represents the reward value. 
We observe that each SK performs well on its corresponding task, indicating that the SK has been well-trained. 
In all cases, CARoL demonstrates a faster convergence speed compared to other methods. This verifies CARoL's capability to efficiently leverage existing knowledge and quickly adapt to the target task. In terms of the final reward, CARoL generally achieves the best performance. Specifically, when the target environment matches one of the source environments, as in subfigures (b, d, g), CARoL produces results comparable to the well-trained SK policies.
When compared to PD, which indiscriminately fuses SK policies, CARoL can prioritize relevant SKs, leading to better performances in (a, c). Additionally, CARoL exhibits a more stable training process than PD. %suffers from significant oscillations, as observed in (a, c) and middle parts of (b, e, f, g).

The LfS uses the same parameter settings as CARoL. LfS struggles to converge in most tasks within the given training steps, whereas CARoL adapts significantly faster. 
Regarding MAML, despite extensive testing meta-training and adaptation, its performance remains poor. This may be due to an undesirable meta-model that is difficult to generalize effectively to new environments. %


\begin{table}[]
    \caption{Contextual similarities - CarRacing.}
    \label{tab:carracing_weights}
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l|c|c|c|c|c|c|c|c}
    \toprule
 $\mu$     & a: 0.2 & b: 0.5 & c: 0.7 & d: 1.0 & e: 1.3 & f: 1.7 & g: 2.0 & h: 2.3 \\
 \midrule 
$\mathbf{T}_1$ &  1.00      & 0.98    & 0.83    &  0.05   & 0.10    &  0.06   & 0.06    & 0.88    \\
$\mathbf{T}_2$ &   0.00     &  0.02   & 0.17    &  0.94   & 0.64    & 0.15    &  0.11   & 0.13    \\
$\mathbf{T}_3$ &   0.00     &   0.00  & 0.00    &  0.01   & 0.26    & 0.79    & 0.83    & 0.79 \\
       \bottomrule
    \end{tabular}}
    \vspace{-1.5em}
\end{table}

%By observing the LfS results, we see that under the same parameter settings as CARoL, LfS struggles to converge in most of the tasks within the given training steps, where as CARoL converges significantly faster. Furthermore, LfS has a clear trend of training efficient, where the more challenging tasks (low environment friction) is more difficult to converge. This is because cars are more easily off-track during the exploration. This issue does not apply to CARoL. Finally, for MAML, we remark that although we performed significant training for the meta-model, the adaptation performance is poor in almost all cases, this might be due to overfitting to the meta-training tasks that fails to generalize or due to poor exploration of the new task.





%When comparing with MAML, we observe that even with the same learning rate and training steps in the inner-loop as SK training, and despite multiple outer-loop iterations, the resulting meta-policy still fails to adapt to new tasks. While the meta-policy provides a good initialization, leading to a strong initial reward during adaptation, it struggles to adjust to the new task in the later stages, causing a noticeable decline in reward performance.


%Comparing the final convergence of CARoL, we find that for target tasks where the friction exceeds the upper and lower boundaries set by the source tasks, the SK corresponding to low/high friction also achieves higher rewards than CARoL. However, for target tasks with friction values in between the low and high friction settings, CARoL converges to a slightly better reward than the SKs. We attribute this to the fact that, in tasks constrained by a single context, the SK trained on the friction boundary provides the most beneficial prior knowledge when the target task exceeds the high or low boundary. In contrast, the remaining two SKs models may negatively impact CARoL’s adaptation. However, for target tasks with intermediate friction values, CARoL can leverage useful learning information from all SKs to adapt more effectively to the new environment.

%When comparing with other baselines, we observe that CARoL generally exhibits faster convergence and higher final reward values. From the LfS results, we see that under the same parameter settings as CARoL, LfS struggles to obtain a feasible policy for challenging tasks, such as environments with low frictions. Additionally, LfS fails to achieve convergence in most of the other tasks within the given training steps. 

%We believe that given sufficient training steps, LfS could eventually converge to a higher reward than CARoL due to its interaction-based learning approach. However, in the context of rapid adaptation to new tasks, LfS is clearly insufficient. Compared to PD, CARoL demonstrates greater stability and faster convergence. Specifically, in subfigure (a), (c), (d), (g), CARoL achieves a higher final reward, while in tasks (a), (b), (d), (e), (f), (g), CARoL converges faster. \XW{Zechen: I cannot explain why PD in (b) can go up even exceed the low friction SK1 so much?} We argue that PD is less effective than CARoL when handling target tasks that were not seen in the source tasks. Unlike CARoL, which performs context-aware adaptation with a bias toward relevant SK, PD simply fuses all SKs indiscriminately. When comparing with MAML, we observe that even with the same learning rate and training steps in the inner-loop as SK training, and despite multiple outer-loop iterations, the resulting meta-policy still fails to adapt to new tasks. While the meta-policy provides a good initialization, leading to a strong initial reward during adaptation, it struggles to adjust to the new task in the later stages, causing a noticeable decline in reward performance.

% CARoL shows faster and higher reward convergence compared to the baselines. 
% Subfigures (b), (d), and (g) correspond to scenarios where the target task is identical to one of the source tasks. In these cases, we observe that each source policy performs optimally on its respective source task. 
% % By prioritizing the most contextually similar knowledge, CARoL achieves comparable accumulated rewards, as seen in (a), (b), and (d). 
% The slight gap in CARoL can be explained by the weight assigned to corresponding source task is not exactly 1. By adapting more knowledge from less relevant source tasks, the performance slightly drops. 
% We can observe that when the friction is lower or higher than the boundaries of our defined low and high limits, the source policy corresponding to either low or high outperforms CARoL. This is because, although CARoL can quickly prioritize the best source knowledge for adaptation, it also considers the similarity of the other source knowledge in the unknown environment. Consequently, the poor performance of the remaining two source knowledge sources adversely impacts the adaptation performance.
% However, when the friction takes a middle value, CARoL performs better in adaptation, achieving a higher reward compared to the source policies. This is because, with the friction at a middle value, the task in this environment is unseen by any individual source policy. Nevertheless, CARoL can integrate all source knowledge and leverage the contextual similarity of the environment to adapt quickly by assigning weights, thereby obtaining a policy.

% In comparison with baselines, we see that PD exhibits a consistently lower reward convergence than CARoL across most target tasks. This is because PD focuses solely on knowledge fusion without considering contextual similarity for new tasks. The convergence reward values of PD in cases (a), (c), and (d) are even lower than CARoL.
% Comparing LfS to CARoL, we observe that LfS demonstrates a significantly slower convergence speed, particularly for (a), (b), and (c). Its reward fails to converge in the same timesteps.
% This is because Lfs has the same network size as CARoL but cannot leverage prior knowledge. Thus, the training is data-demanding and convergence is difficult, especially in cases with lower friction. In CarRacing, a significant low friction environment is very difficult for RL training.
% It is worth noting that in target tasks (g) and some trials of (h),  LfS achieves higher rewards than CARoL. This is because the source task may not provide sufficient useful knowledge to the target tasks. In these cases, LfS benefits from learning new knowledge from the new task and thus outperforms CARoL.

\subsection{Simulated Experiment: LunarLander}
\subsubsection{Experiment Setup}
As shown in Fig. \ref{fig:sim_intro}-(b) LunarLander is a control task where an autonomous lander robot must safely land on a designated landing pad in a simulated lunar environment. The robot must balance thrust and control to achieve a smooth landing while minimizing fuel consumption.
The LunarLander environment allows adjustments of gravity and wind power. For source tasks, we set the two parameters as $(-5, 0)$; $(-10, 0)$; $(-5, 10)$; $(-10, 10)$, respectively.
To implement CARoL, we obtain all source knowledge using TD3 (Twin Delayed Deep Deterministic)~\cite{fujimoto2018addressing}. 
    The source knowledge is represented as pre-trained source policies and state-action value functions. Therefore, our CARoL utilize Algorithm \ref{Alg_AC} for adaptation on the target tasks. Here, we consider the actor and critic with equal importance, i.e., $\beta=1$.
\begin{comment}
\begin{itemize} [leftmargin=*]
    \item The observation space is an 8-dimensional vector representing the lander’s position, velocity, angle, and contact sensors for the landing legs.

    \item The continuous action space determines the throttle percentage of the vertical main engine $[-1, 1]$, and the throttle of the lateral boosters $[-1, 1]$. 
    %\marginXW{I don't understand, why the virtual throttle can be negative. Zechen: Throught OpenAI's explanation, the main engine will be turned off completely if main < 0 and the throttle scales affinely from 50 percent to 100 percent for 0 <= main <= 1; if -0.5 < lateral < 0.5, the lateral boosters will not fire at all. If lateral < -0.5, the left booster will fire, and if lateral > 0.5, the right booster will fire.}

    \item Positive rewards are given for a smooth landing, and penalties are applied for crashes, excessive fuel consumption, and staying off the designated landing pad. 
\end{itemize}


The LunarLander environment allows adjustments of gravity and wind power, based on which we can create different source and target tasks. 
Different gravity levels, $g \in [-12, -2]$,
affect the vertical force on the lander robot, while varying wind power, $F_w \in [0, 10]$, impacts the horizontal force\footnote{In our experiments, wind power is modeled as a time-invariant fixed value to emphasize its impact on state transitions. This differs from the standard environment, where wind power is randomized at each time step.}.
The configuration of source tasks and target tasks for this experiment is visualized in Fig.~\ref{fig:lunarlander_config}. The horizontal axis represents gravity, the vertical axis represents wind power. They together expand a 2-D configuration space. The blue dots indicate the source tasks, which are defined as follows: $(-5, 0)$; $(-10, 0)$; $(-5, 10)$; $(-10, 10)$. The red crosses represent the target tasks used for testing. These target tasks are located above, to the left, to the right, and inside a square formed by the source tasks over the configuration space. 
Note that the environment configurations for both source and target tasks are unknown to the robot. Using context awareness, the robot will derive a unique prioritization of source knowledge for each target task.


%\marginXW{Also Mark a-j of target tasks? Zechen: Changed. Please check.}


\smallskip
\subsubsection{Implementation of CARoL and other Baselines}
\begin{itemize} [leftmargin=*]
    \item \textbf{CARoL}: In LunarLander, we obtain all source knowledge using TD3 (Twin Delayed Deep Deterministic)\cite{fujimoto2018addressing}. 
    The source knowledge is represented as pre-trained source policies and state-action value functions. Therefore, our CARoL utilize Algorithm \ref{Alg_AC} for adaptation on the target tasks. Here, we consider the actor and critic with equal importance, i.e., $\beta=1$
    
    %To demonstrate the generality of the CARoL algorithm, the source knowledge in this case is represented by pre-trained source actors and source critics, where the critics are state-action value functions. Therefore, our CARoL utilizes Algorithm \ref{Alg_AC} for adaptation on the target tasks.
    % First introduce that the knowledge is obtained using TD3 (Twin Delayed Deep Deterministic)\cite{fujimoto2018addressing}. 
    % What is the knowledge? -> We use Alg 3...

    \item \textbf{CARoL+}: The implementation of CARoL+ incorporates CARoL's loss function~\eqref{eqa:lossAC} and a standard TD3 learning loss. As explained in Remark~\ref{RM1}, this facilitates knowledge adaptation not only through CARoL but also via reward-based learning from the environment.
    
    
    
    %The implementation of CARoL+ builds upon the loss function of CARoL by incorporating the TD3 learning loss. While optimizing the adaptation loss \eqref{eqa:lossAC}, it also integrates interaction learning between CARoL and the environment through reward-based learning.

    \item \textbf{Other baselines that have been introduced in CarRacing}\footnote{In this part, MAML is excluded due to its poor performance in the CarRacing and the excessively long training time of the meta-policy.}: For all other baselines, we use TD3 to obtain the source knowledge, and their network architectures are kept consistent with the target actor initialized in CARoL. 
\end{itemize}
\textbf{Implementation Details}: 
    For training SKs, we use a fully connected actor network, consisting of the architecture with a 4-layer MLP with layer sizes
    \{96, 192, 96, 2\}
    % ($96 \rightarrow 196 \rightarrow 96$) 
    and ReLU activations in the hidden layers, followed by a tanh activation in the output layer. 
    The critic network uses the same architecture. 
    For context awareness of CARoL, we use the same network in CarRacing for state transition functions. The input consists of observed state and the executed action, and its output is the next observed state.
    For CARoL, CARoL+, PD, and LfS, we use the same but lighter actor and critic networks, i.e., 
    \{48, 96, 48, 2\}.
    % ($48 \rightarrow 98 \rightarrow 48$). 
    All methods are trained using AdamW with a fixed learning rate of $4 \times 10^{-4}$ and a discount factor $0.98$. The number of total training episodes for SKs is 15,000 episodes with a maximum of 1,000 steps per episode while others are 10,000 episodes with a maximum of 500 steps per episode. 
% \marginXW{Critic?}
    % \item \textbf{Parameters}: Note that the neural network structures used by XX are the same. \XW{add here.}


% \noindent$\bullet$ {CARoL}: First introduce that the knowledge is obtained using TD3 (Twin Delayed Deep Deterministic)\cite{}. 
% What is the knowledge? -> We use Alg 3...

% \noindent$\bullet$ {CARoL+}:

% \noindent$\bullet$ {Other baselines that are not introduced in CarRacing}:
\end{comment}

\begin{comment}
\captionsetup[subtable]{position=above}

\begin{table}
\footnotesize
  \centering
  \caption{shared caption for all three subtables}
  \begin{subtable}[t]{0.45\linewidth}
    \caption{Contextual similarities - CarRacing.}
    \label{tab:carracing_weights}
    \centering
    \begin{tabular}{l|ccc}
    \toprule
    & $\mathbf{T}_1$ & $\mathbf{T}_2$ & $\mathbf{T}_3$ \\
    \midrule 
       \text{a: }$\mathbf{\mu=0.2}$  & 1.00 & 0.00 & 0.00 \\
       \midrule 
       \text{b: }$\mathbf{\mu=0.5}$  & 0.98 & 0.02 & 0.00 \\
       \midrule 
       \text{c: }$\mathbf{\mu=0.7}$  & 0.83 & 0.17 & 0.00 \\
       \midrule 
       \text{d: }$\mathbf{\mu=1.0}$   & 0.05 & 0.94 & 0.01 \\
       \midrule 
       \text{e: }$\mathbf{\mu=1.3}$   & 0.10 & 0.64 & 0.26 \\
       \midrule 
       \text{f: }$\mathbf{\mu=1.7}$  & 0.06 & 0.15 & 0.79 \\
       \midrule 
       \text{g: }$\mathbf{\mu=2.0}$   & 0.06 & 0.11 & 0.83 \\
       \midrule 
       \text{h: }$\mathbf{\mu=2.3}$   & 0.08 & 0.13 & 0.79 \\
       \bottomrule
    \end{tabular}
  
    
  \end{subtable}
  \begin{subtable}[t]{0.45\linewidth}
    \caption{Contextual similarities - LunarLander.}
    \label{tab:lunarlander_weights}
    \centering
    \begin{tabular}{l|cccc}
    \toprule
         & $\mathbf{T}_1$ & $\mathbf{T}_2$ & $\mathbf{T}_3$ & $\mathbf{T}_4$\\
         \midrule 
       \text{a: }\textbf{(-5, 0)}  & 0.95 & 0.05 & 0.00 & 0.00\\
       \midrule 
       \text{b: }\textbf{(-10, 0)}  & 0.01 & 0.98 & 0.00 & 0.01\\
       \midrule 
       \text{c: }\textbf{(-5, 10)} & 0.06 & 0.01 & 0.91 & 0.02\\
       \midrule 
       \text{d: }\textbf{(-10, 10)}   & 0.00 & 0.01 & 0.01 & 0.98\\
       \midrule 
       \text{e: }\textbf{(-3, 2)}   & 0.62 & 0.09 & 0.28 & 0.01\\
       \midrule 
       \text{f: }\textbf{(-6, 9)}   & 0.09 & 0.00 & 0.81 & 0.10\\
       \midrule 
       \text{g: }\textbf{(-9, 5)}   & 0.19 & 0.37 & 0.18 & 0.26\\
       \midrule 
       \text{h: }\textbf{(-7, 0)}   & 0.35 & 0.34 & 0.22 & 0.09\\
       \midrule 
       \text{i: }\textbf{(-11, 9)}   & 0.01 & 0.12 & 0.10 & 0.77\\
       \midrule 
       \text{j: }\textbf{(-8, 12)}   & 0.13 & 0.17 & 0.29 & 0.41\\
       \bottomrule
    \end{tabular}
  \end{subtable}
\end{table}

\end{comment}

\setlength{\tabcolsep}{3pt}
\begin{table}[]
    \caption{Contextual similarities - LunarLander.}
    \label{tab:lunarlander_weights}
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c}
    \toprule
  & a:  & b:  & c:  & d:  & e: & f:  & g: & h: & i: & j: \\
  & (-5, 0) & (-10, 0) &  (-5, 10) & (-10, 10) &  (-3, 2) & (-6, 9) & (-9, 5) & (-7, 0) &  (-11, 9) &  (-8, 12) \\
 \midrule 
$\mathbf{T}_1$ &  0.95    & 0.01& 0.06    &  0.00   & 0.62    &  0.09   & 0.19    & 0.35 &0.01&0.13   \\
$\mathbf{T}_2$ &   0.05   &  0.98 & 0.01    &  0.01   & 0.09    & 0.00    &  0.37   & 0.34 &0.12&0.17   \\
$\mathbf{T}_3$ &   0.00   & 0.00  & 0.91    &  0.01   & 0.28    & 0.81    & 0.18    & 0.22&0.10&0.29 \\
$\mathbf{T}_4$ &   0.00   &0.01  & 0.02    &  0.98   & 0.01    & 0.10    & 0.26    & 0.09&0.77&0.41 \\
       \bottomrule
    \end{tabular}}
    \vspace{-1em}
\end{table}

\begin{comment}
\begin{table}[]
    \caption{Contextual similarities - LunarLander.}
    \label{tab:lunarlander_weights}
    \centering
    \begin{tabular}{l|cccc}
    \toprule
         & $\mathbf{T}_1$ & $\mathbf{T}_2$ & $\mathbf{T}_3$ & $\mathbf{T}_4$\\
         \midrule 
       \text{a: }\textbf{(-5, 0)}  & 0.95 & 0.05 & 0.00 & 0.00\\
       \midrule 
       \text{b: }\textbf{(-10, 0)}  & 0.01 & 0.98 & 0.00 & 0.01\\
       \midrule 
       \text{c: }\textbf{(-5, 10)} & 0.06 & 0.01 & 0.91 & 0.02\\
       \midrule 
       \text{d: }\textbf{(-10, 10)}   & 0.00 & 0.01 & 0.01 & 0.98\\
       \midrule 
       \text{e: }\textbf{(-3, 2)}   & 0.62 & 0.09 & 0.28 & 0.01\\
       \midrule 
       \text{f: }\textbf{(-6, 9)}   & 0.09 & 0.00 & 0.81 & 0.10\\
       \midrule 
       \text{g: }\textbf{(-9, 5)}   & 0.19 & 0.37 & 0.18 & 0.26\\
       \midrule 
       \text{h: }\textbf{(-7, 0)}   & 0.35 & 0.34 & 0.22 & 0.09\\
       \midrule 
       \text{i: }\textbf{(-11, 9)}   & 0.01 & 0.12 & 0.10 & 0.77\\
       \midrule 
       \text{j: }\textbf{(-8, 12)}   & 0.13 & 0.17 & 0.29 & 0.41\\
       \bottomrule
    \end{tabular}
\end{table}
\end{comment}

\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth]{Contents/Figures/reward_lunarlander_v2.pdf}
    \caption{Comparison of cumulative reward for CARoL and baselines under different LunarLander tasks. The x-axis represents the running episodes and the y-axis represents the reward. The height of dash lines demonstrates the average accumulative reward of source knowledge (SK) under the task.}
    \vspace{-1em}
    \label{fig:lunarlander_reward}
\end{figure*}

\smallskip
\subsubsection{Results and Analysis}

Table \ref{tab:lunarlander_weights} presents the contextual similarity weights learned for four source tasks in different target tasks under the LunarLander simulated experiment. Similar to the CarRacing, we observe that the weight is negatively correlated with their geometric distance in the figure. We also provide a sanity check here as the first four rows of the table correspond to the same scenarios as source tasks. We can observe a similar pattern to CarRacing. 
Meanwhile, by reading the exact values in the table, we also note that the relationship between weights and distances is not strictly proportional, because the impact from environmental configurations to context (state transition) is nonlinear. %For instance, different combinations of gravity and wind power may lead to similar state transitions. Then, the contextual similarity allows the corresponding prior knowledge to be effectively adapted.

Fig.~\ref{fig:lunarlander_reward} shows the reward curves, where the x-axis represents the number of learning episodes, and the y-axis represents the reward value. CARoL shows faster and higher reward convergence compared to the baselines. 
Subfigures (a-d) correspond to scenarios where the target task is identical to one of the source tasks. In these cases, we observe that each source policy performs best with the highest evaluation reward on its respective source task. 
%By prioritizing the most contextually similar knowledge, CARoL achieves comparable accumulated rewards, as seen in (a), (b), and (d). 
%For (c), the slight gap of CARoL can be explained by the third row of Table~\ref{tab:lunarlander_weights}, where the weight assigned to $\mathbf{T}_3$ is not as close to 1 as in other cases. By adapting more knowledge from less relevant source tasks, the performance slightly drops. 
Across all other target tasks, where the target is different from any source task, we observe that the average reward of any single source policy is consistently lower than that of CARoL. This is because the source policies lack experience with the target task’s specific contexts. %CARoL, on the other hand, effectively combines source knowledge based on contextual similarity, allowing it to achieve better performance.

In comparison with baselines, similar to the observations in CarRacing, we see that PD exhibits a consistently lower reward convergence than CARoL across most target tasks. %This is because PD focuses solely on knowledge fusion without considering contextual similarity for new tasks. 
%Both PD and CARoL exhibit some training-phase oscillations in the early stages when initially incorporating knowledge from multiple source policies. Nevertheless, these oscillations diminish as the adaption process progresses. 
Comparing LfS to CARoL, we observe that LfS demonstrates a significantly slower convergence speed, particularly for (f) and (h), and generally achieves lower final rewards.
This is because Lfs has a same network size as CARoL but cannot leverage prior knowledge. %Thus, the training is data-demanding and the convergence is difficult. 
It is worth noting that in target tasks (i) and some trials of (j),  LfS achieves higher rewards than CARoL. This is because the source task may not provide sufficient useful knowledge to the target tasks, as these target tasks use parameters outside the combination of the source tasks. In these cases, LfS benefits from learning new knowledge from the new task and thus outperforms CARoL.

However, this issue can be addressed by CARoL+ (cf. Sec. \ref{sec_Carol+}). CARoL+ integrates interaction-based learning during adaptation, allowing it to achieve the highest reward across all cases. This compensates for CARoL’s potential limitations in final convergence values. Additionally, CARoL+ retains CARoL’s advantage of fast convergence while also being the most stable one during the convergence process. 

% \marginXW{Add CARoL+ results. 
% CARoL+ should be CARoL add a regular RL loss for model updates.
% Add meta-learning as baseline.
% After adding these, some analyses will need to be rewritten.
% }

%within the range. Additionally, we only considered one wind direction, as we believe that wind in the opposite direction would merely reverse the control effects on the robot.}. %Let $g$ denote the gravity ($g \in [-12, -2]$) and $F_w$ denote the wind power ($F_w \in [0, 10]$) \footnote{In the original LunarLander platform, wind power is randomly selected within the range. However, in our experiments, we hardcode wind power to a selected fixed value within the range. Additionally, we only considered one wind direction, as we believe that wind in the opposite direction would merely reverse the control effects on the robot.}.
%We also varied the distances between the target tasks and the source tasks in the figure to observe the impact of task similarity on performance based on their geometric distance. %Here, we use the combined vector of observations and actions as the features for training the state transition function.
% \marginXW{Table captions are on top of the tables.}
%Furthermore, the average accumulated reward achieved by these teacher knowledge on their respective source tasks is generally comparable to the final reward value to which CARoL converges, as seen in (a), (b), and (d). In some cases, such as (c), the teacher knowledge even slightly outperforms CARoL. This occurs because, as shown in the table, CARoL identifies that the current task context is almost identical to the corresponding source task and therefore adapts nearly entirely to the teacher knowledge for that source task. However, in cases like (c), CARoL also considers other teacher knowledge, and particularly Teacher 4, which does not perform well in this environment, leading to a slight impact on the adaptation results. Across all target tasks, we can see that the average reward of any single teacher knowledge is consistently lower than that of CARoL. This is because these teacher knowledge have not encountered the target task's corresponding contexts. CARoL, on the other hand, effectively combines all teacher knowledge based on context similarity, allowing it to achieve superior performance.


%these target tasks use parameters outside the box of the source task (cf. )

%cannot be directly measured to determine which has a greater impact on task dynamics. As a result, the similarity ratio between tasks cannot be directly inferred from their geometric distances. %Therefore, we still rely on a context-aware module and a similarity module to compute the similarity weights.

%Fig. \ref{fig:lunarlander_reward} shows the reward curves for the LunarLander experiment, where the x-axis represents the number of learning episodes, and the y-axis represents the reward value. It can be observed that CARoL achieves faster and higher reward convergence compared to the baselines overall. Subfigures (a-d) present comparisons between CARoL and baselines on the source tasks. From these plots, we observe that each teacher knowledge performs optimally on its corresponding source task and can be clearly distinguished from the test performance of other teacher knowledge. Furthermore, the average accumulated reward achieved by these teacher knowledge on their respective source tasks is generally comparable to the final reward value to which CARoL converges, as seen in (a), (b), and (d). In some cases, such as (c), the teacher knowledge even slightly outperforms CARoL. This occurs because, as shown in the table, CARoL identifies that the current task context is almost identical to the corresponding source task and therefore adapts nearly entirely to the teacher knowledge for that source task. However, in cases like (c), CARoL also considers other teacher knowledge, and particularly Teacher 4, which does not perform well in this environment, leading to a slight impact on the adaptation results. Across all target tasks, we can see that the average reward of any single teacher knowledge is consistently lower than that of CARoL. This is because these teacher knowledge have not encountered the target task's corresponding contexts. CARoL, on the other hand, effectively combines all teacher knowledge based on context similarity, allowing it to achieve superior performance.

%In the comparison with baselines, similar to the observations in CarRacing, we can see that the issue with PD lies in its reward convergence being consistently lower than CARoL across most target tasks. This is because multi-task RL in PD focuses solely on the knowledge fusion process without considering adaptation to new tasks. In contrast, CARoL effectively combines knowledge fusion with proper adaptation to the new task. However, we observe that both PD and CARoL exhibit some training-phase oscillations in the early stages. This occurs because, during the initial phase of knowledge fusion, certain source task strategies may not be applicable to the target task. Nevertheless, such oscillations typically diminish as the fusion stabilizes. Comparing LfS to CARoL, we observe that LfS demonstrates a much slower convergence trend. In some cases, such as (f) and (h), LfS does not fully converge within the predefined number of episodes in the experimental setup. Additionally, since LfS is configured to have the same network size as CARoL, its final reward values are lower than CARoL in most cases. Although LfS achieves higher convergence rewards in target tasks (d) and (i), we can still conclude that, with comparable network sizes, CARoL's adaptation ability surpasses LfS due to its effective utilization of prior knowledge.

\subsection{Real World: Ground vehicle Off-road Navigation}
We apply CARoL to an off-road mobility problem with a physical robot. As shown in Fig. \ref{fig:sim_intro}-(c), the goal is to enable the robot to autonomously and successfully navigate from the start to the goal. RL for real-world off-road mobility is particularly inefficient due to the prohibitive cost of collecting physical vehicle-terrain interaction data. Therefore, in this experiment, we aim to apply CARoL to adapt policies learned in simulation to the real world. 

\subsubsection{Experiment Setup}
We leverage a high-fidelity multi-physics simulator,  Chrono~\cite{tasora2016chrono}, to train two different off-road navigation policies: SK1 for concrete terrain and SK2 for grass terrain. We generate off-road terrain with undulating topographies and vary the friction coefficient between the vehicle tires and the underlying terrain, i.e., 0.9 and 0.4. 
Here, different friction levels influence traversability. For example, for the same slope, friction determines whether the robot can climb it or must bypass it.
% \marginXW{Hi Tong or Xuesu, double check if the revision makes sense.}
In the real world, we construct an off-road mobility testbed with hundreds of rocks and boulders. We posit the friction coefficient of the real-world rocks and boulders to be between 0.57 and 0.73, necessitating adaption from the two SKs into a new policy. 

\begin{comment}
    

\begin{itemize} [leftmargin=*]
\item The observation space encompasses a 16-dimensional terrain encoding (derived from elevation footprints via a SWAE~\cite{kolouri2018sliced} architecture), normalized heading error, and current speed. 

\item The action space consists of continuous speed and steering commands.

\item The robot receives rewards for moving towards the goal and penalties for large roll and pitch angles, which are indicators of the robot’s stability during navigation.
\end{itemize}
\end{comment}

\subsubsection{Implementation of CARoL}
In the simulators, similar to CarRacing, we use PPO to train two source knowledge policies from scratch and train state transition functions for each environment as context representation.
To implement CARoL in the real-world environment, we first compute the contextual similarity. To achieve this, we manually control the vehicle to randomly navigate 20 trials on the real-world off-road terrain to collect trajectory data, instead of relying on random exploration, for real-world sample efficiency.
The contextual similarity is quantified by comparing the prediction errors of the source task transition functions over trajectories collected in the real-world environment.

Based on the obtained contextual similarity and source task policies, we employ CARoL-Algorithm \ref{Alg_policy} to adapt to the real world. %Since the adaptation is on-policy, we iteratively collect trajectories using the current policy and update the policy with the collected data. 
%The policy model is implemented as a 3-layer fully-connected network with hidden layers$\{32, 32, 2\}$ using ReLU activations. we use the Adam optimizer with a fixed learning rate of $1\times 10^{-3}$. The discount factor is set to 0.99. 
We perform a total of 10 iterations with 8 navigation trials each (approximately 130 minutes in total), during which the vehicle gradually improve from initially failing (veering off the experimental field, getting stuck halfway, or flipping over) to successfully reaching the goal. 
In the final two iterations, the vehicle successfully reaches the goal in every episode, indicating a good adaptation performance. We then compare this converged model with the source knowledge policies.
We do not implement baseline methods due to the prohibitive cost of collecting extensive physical vehicle-terrain interaction data. For the same reason, we do not employ CARoL+.


\subsubsection{Experiment Results and Analysis}
In the comparison experiments, each model undergoes five trials from the start to the goal. The source knowledge refers to the model trained in the Chrono simulator, which is directly deployed on the robot. The evaluation metrics for this experiment, aligned with the RL rewards, include success rate, roll, and pitch. While traveling time is not evaluated, it is provided as a reference.

As shown in the results Table \ref{tab:physical_results}, CARoL achieves the highest success rate, and the robot demonstrates the most stable navigation under CARoL’s adapted model. Although CARoL takes the longest time to reach the goal, this is expected, as we do not impose any reward or penalty on travel time in this task. The longer duration might suggests that the robot is carefully selecting paths based on traversability.
The primary objective is to ensure that the robot autonomously reaches the goal successfully, and CARoL’s high stability in terms of roll and pitch plays a crucial role in achieving this outcome. SK2, trained on the low friction grass terrain, achieves the shortest traveling time thanks to the increased friction of the real-world rocks and boulders. 



%The policy model in CARoL, implemented as a series of fully-connected layers with $\{32, 32\}$ neurons and ReLU activations, successfully learns to emulate a weighted adaptation of source behaviors through our framework, where the weights are determined by the relevance evaluation during context awareness from the state transition comparison. We train the transition functions in simulator by a 3-layer MLP \{18, 32, 32, 16\} with ReLU activations. 
%\marginXW{Tong: I doubt that 16 terrain embedding can represent the friction info from real world or not? Xuan; How it is suggested by the experiment?} 
%The similarity between tasks is quantified by comparing the prediction errors of source transition functions on trajectories from the target environment, enabling CARoL to adaptively weigh the knowledge adapted from each source knowledge. 


%Similar to the CarRacing simulation, the source knowledge here is represented as source policies and our CARoL then use Algorithm \ref{Alg_policy} for adaptation to the real world task. 


%During CARoL's adaptation, we use the Adam optimizer with a fixed learning rate of $1\times 10^{-3}$ to accelerate convergence. The discount factor is set to 0.99. 


%Before the adaptation begins, we manually control the vehicle to randomly navigate 20 times from the start to the goal direction on off-road terrain to collect trajectory data. The similarity between tasks is quantified by comparing the prediction errors of source transition functions on trajectories from the target environment. Based on the obtained relevance, we learn from the source knowledge. However, since the adaptation is on-policy, we need to iteratively collect trajectories using the current policy and update the policy with the collected data. We perform a total of 10 iterations, during which the vehicle gradually improves from initially failing (veering off the experimental field or flipping over) to successfully reaching the goal. 


 





%\XW{Do we need to explain why we did not include other baselines in the physical experiments?}

% This approach utilizes KL-divergence minimization between teacher-student policy distributions with transition dynamics matching, resulting in a compact student policy that can effectively generalize across different environmental conditions while maintaining the essential behaviors of the specialized teacher policies.

% \XW{detailed parameters for learning, network size, etc.}

% \XW{Analysis... }

\begin{table}
\caption{Physical Experiment Results.}
% Best results are shown in bold.} 
\centering
\resizebox{\columnwidth}{!}{%
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{c|c|cc|ccccc}
\toprule
                                          % & \multicolumn{3}{c}{\footnotesize {V4W}}                        \\
%\cmidrule(rl){1-2} \cmidrule(rl){3-4} \cmidrule(rl){5-6}
% \cmidrule(l){2-4} 
Method & {Success $\uparrow$} &  {Roll $\downarrow$} & {Pitch $\downarrow$} & {Time (no penalty)} \\
\midrule
CARoL & {\textbf{5/5}} & \textbf{{4.08}\textdegree$\pm$4.65\textdegree} & \textbf{{8.55\textdegree$\pm$5.13}\textdegree} &{16.88s$\pm$1.97s} \\
SK1 & 3/5 & {5.44}\textdegree$\pm$7.13\textdegree & {10.35}\textdegree$\pm$5.29\textdegree & {11.78s$\pm$1.44s}\\
SK2 & 2/5 & {5.75}\textdegree$\pm$5.00\textdegree & {8.61}\textdegree$\pm$5.12\textdegree & \textbf{8.55s$\pm$0.67s}\\
\bottomrule
\end{tabular}%
}
\vspace{-1.5em}
\label{tab:physical_results}
\end{table}

%\newpage
\begin{comment}
\textbf{CarRacing} as shown in Fig. \ref{fig:sim_intro} (a) is a continuous control task where an autonomous mobile robot must navigate a procedurally generated racetrack to maximize cumulative rewards. The task involves balancing speed and control to avoid going off-track while efficiently covering the racetrack. The observation space of the task is a $96\times 96 \times 3$ RGB image of the top-down view of the car and track. The action space of the task is continuous, consisting of three dimensions: steering $[-1, 1]$, acceleration $[0,1]$, and brake $[0,1]$. The robot receives a reward for visiting track tiles and is penalized for each timestep. The episode terminates when all tiles are visited or the car goes off-track. 

In CarRacing, the dynamic context of the task primarily lies in the friction. We designed three different task environments with low $\mu=0.5$, medium $\mu=1$, and high friction $\mu=2$ in the source tasks. Our experimental goal is to quickly obtain an optimal policy in a target task with an unknown friction level. Additionally, we consider that the images in the observations do not intuitively reflect friction as the dynamic context. Therefore, we select \XW{XXX, XXXX, and XXXX} as features for training the state transition function.

\textbf{LunarLander} as shown in Fig. \ref{fig:sim_intro} (b) is a control task where an autonomous lander robot must safely land a spaceship on a designated landing pad in a simulated lunar environment. The robot must balance thrust and control to achieve a smooth landing while minimizing fuel consumption. We use the continuous version. The observation space is an 8-dimensional vector representing the lander’s position, velocity, angle, and contact sensors for the landing legs. The continuous action space determines the throttle of the main engine $[-1, 1]$ and the throttle of the lateral boosters $[-1, 1]$. Positive rewards are given for a smooth landing, and penalties are applied for crashes, excessive fuel consumption, and staying off the designated landing pad. 

In the LunarLander environment, the contexts that influence task dynamics are more diverse, including gravity, wind power, and turbulence power. In our experiments, we selected gravity and wind power to form our context space. Different gravity levels affect the vertical force on the lander robot, while varying wind power impacts the horizontal force on the lander robot. Let $g$ denote the gravity ($g \in [-12, -2]$) and $F_w$ denote the wind power ($F_w \in [0, 10]$) \footnote{In the original LunarLander platform, wind power is randomly selected within the range. However, in our experiments, we hardcode wind power to a selected fixed value within the range. Additionally, we only considered one wind direction, as we believe that wind in the opposite direction would merely reverse the control effects on the robot.}.
\end{comment}

% \marginXW{mark T1-T4 on the plot.}




%\textbf{Off-road navigation?} \XW{details}

%\subsection{Implementation of CARoL and Baselines}



%\subsection{Overall Results on CarRacing}

%\subsection{Overall Results on LunarLander}





